involve-MI: Informative Planning with High-Dimensional Non-Parametric Beliefs

One of the most complex tasks of decision making and planning is to gather information. This task becomes even more complex when the state is high-dimensional and its belief cannot be expressed with a parametric distribution. Although the state is high-dimensional, in many problems only a small fraction of it might be involved in transitioning the state and generating observations. We exploit this fact to calculate an information-theoretic expected reward, mutual information (MI), over a much lower-dimensional subset of the state, to improve efficiency and without sacrificing accuracy. A similar approach was used in previous works, yet specifically for Gaussian distributions, and we here extend it for general distributions. Moreover, we apply the dimensionality reduction for cases in which the new states are augmented to the previous, yet again without sacrificing accuracy. We then continue by developing an estimator for the MI which works in a Sequential Monte Carlo (SMC) manner, and avoids the reconstruction of future belief's surfaces. Finally, we show how this work is applied to the informative planning optimization problem. This work is then evaluated in a simulation of an active SLAM problem, where the improvement in both accuracy and timing is demonstrated.

==> 2022 Arxiv/00-Abstract.tex <==
\begin{abstract}

One of the most complex tasks of decision making and planning is to gather information. This task becomes even more complex when the state is high-dimensional and its belief cannot be expressed with a parametric distribution. Although the state is high-dimensional, in many problems only a small fraction of it might be involved in transitioning the state and generating observations. We exploit this fact to calculate an information-theoretic expected reward, mutual information (MI), over a much lower-dimensional subset of the state, to improve efficiency and without sacrificing accuracy. A similar approach was used in previous works, yet specifically for Gaussian distributions, and we here extend it for general distributions. Moreover, we apply the dimensionality reduction for cases in which the new states are augmented to the previous, yet again without sacrificing accuracy.
We then continue by developing an estimator for the MI which works in a Sequential Monte Carlo (SMC) manner, and avoids the reconstruction of future belief's surfaces. Finally, we show how this work is applied to the informative planning optimization problem.
This work is then evaluated in a simulation of an active SLAM problem, where the improvement in both accuracy and timing is demonstrated.

% TODO: We use the $\rho$-POMDP formulation

\end{abstract}

==> 2022 Arxiv/02-Related.tex <==
%\add{The problem we address in this paper involves two different literature communities: the estimation community and the decision making and planning community. The estimation community provides many estimators for information-theoretic rewards, each with its own advantages and disadvantages, as can be seen for example in \cite{beirlant1997nonparametric}. The decision making community usually uses these estimators while making assumptions and approximations.}

The notion that in some cases the correlations between some of the state variables could be discarded for the calculation of entropy, thus improving the efficiency, was first introduced in \cite{Indelman16ral}. This idea was extended to a more general case in \cite{Elimelech17icra} and \cite{Kopitkov17ijrr}. However, these papers addressed the problem assuming Gaussian distributions. The current paper extends these works to the non-parametric case.

Reviewing state-of-the-art approaches for planning with non-parametric beliefs, most do not attempt to address the problem of evaluating the uncertainty of a state (e.g. \cite{Kurniawati08rss}, \cite{Silver10nips}, \cite{Ye17jair}, \cite{Kurniawati16chapter}).
% TODO: \add{
These works consider the POMDP framework, which does not support belief-dependent rewards. The recent approaches presented in e.g. \cite{Sunberg18icaps} and \cite{Fischer20icml},
% \GR{(and \cite{Garg19rss}?)}
do support belief-dependent rewards, by using the more general $\rho$-POMDP framework.
%and simulating particle sets in a MCTS fashion to construct a search tree. 
Yet, while these are concerned with improving the search over a tree, the calculation of the information-theoretic costs when the state is high-dimensional remains a problem.
% TODO: }
% yet it is not concerned with the dimension of the state and does not try to address this issue.

% TODO: \add{[need to reformulate]:
Many estimators exist for information-theoretic rewards. A brief overview of the most common estimators for entropy can be found in \cite{Beirlant97jmss}.
% TODO: [Talk about re-substitution with KDE].
Another approach to estimate entropy, a particle-filter based approach, is presented in \cite{Boers10fusion}.
% TODO: [in what context?].
Furthermore, \cite{Ryan08gnc} suggests to use a piece-wise linear approximation of the beliefs' surface.
% TODO: [in the context of planning?].
Yet, all will face the Curse of Dimensionality. The work presented in \cite{Stowell09spl} claims to support high-dimensional spaces, however the simulations show this approach isn't superior for any arbitrary belief compared to other approaches.
% TODO: }

% TODO: \add{[need to reformulate]: When changing the context a bit, and looking at an expected reward, mutual information, \cite{Chli09thesis} and \cite{zhang2020fsmi}}
When changing the context a bit, and looking at an expected reward, mutual information, \cite{Chli09thesis} and \cite{Zhang20ijrr} both state that the MI over a multi-dimensional variable can be calculated over a lower dimensional subset of this variable. Yet their statements are applied specifically for the problems of feature matching and active mapping, respectively. %Also, they do not consider what happens if the state is changed.
Also, these do not address problems in which quantifying the information should also take into account the state might change.

% TODO: \add{Information theory: \cite{Cover91book} [Does it contain what we prove about MI?], Non-Gaussian: \cite{Pathak18ijrr}, Monte Carlo Methods: \cite{doucet2001sequential}, Inference: \cite{Montemerlo02aaai} (FastSLAM), \cite{Montemerlo03ijcai} (FastSLAM 2.0), \cite{Fourie16iros} (Fourie), \cite{Sudderth10acm} (Nonparametric belief propagation), \cite{huang2021nf} (nonparametric iSAM 2)}

%TODO: Look again how we differ from the article with the entropy estimation with the factors (in terms of dimensionality)


%To the best of our knowledge, the only work which claims to support high-dimensional non-parametric state-spaces in the context of informative planning is the approach introduced in \cite{Platt11isrr}. It uses a cost other than entropy, defined as the distance between the ML observations acquired in the hypothesis state to the ML observations acquired in other sampled instances of the state. The larger the distance between these observations, the higher chance we will have to distinguish between the state instances, thus reduce the uncertainty. So, the planner selects the set of actions with the largest distance. This method \GR{(allegedly)} reduces the time complexity to depend only on the number of sampled instances of the state, however to reliably represent the belief, this number by itself should be exponential in the dimension of the state \GR{(Not sure this is true)}. A few more issues arise when using this approach. One such issue is that it considers the same observation variables for each of the state instances, while in the general case each state instance might involve different observation variables (also with different dimensionalities, i.e. one action might induce one observation, while another action might involve multiple observations). \GR{How is this measure different than entropy? Is the ML assumption not good? Update: Let's say that we need to choose between an action which will get us a very noisy observation and an action which will get us a very accurate observation. Platt's approach will choose the action with the noisy action, which is a problem (Still need to check if true, but that's the direction)}

To the best of our knowledge, there are two works which, at some level, construct planners with an information-gathering task and which support high-dimensional non-parametric beliefs with complexity not exponential with the dimension of the state, yet do not support the more general setting we are addressing in this paper. One of which is \cite{Stachniss05rss}, addressing the very specific active SLAM problem. It exploits the unique structure of SLAM to use Rao-Blackwellization, which might not be useful for more general problems. Also, it approximates the joint entropy by averaging the individual entropies of the state variables, thus breaks up the correlations between them.

The second work is \cite{Platt11isrr}, which uses a slightly different and more specific formulation than the general POMDP, where the objective is to minimize the expected cost. In its formulation, the objective is to reach a desired region of the state space with a guaranteed minimum probability of success. This, in turn, means that it wouldn't necessarily choose the most informative path. Also, it does not support, at least directly, information-theoretic rewards. And, lastly, this approach was eventually tested only on problems with up to four dimensions.

Our approach deals with the limitations of the former.

% TODO: \VI{[need to elaborate more; mention also $\rho$-pomdp]}

% TODO: ML assumption

==> 2022 Arxiv/03-ProblemFormulation.tex <==
\subsection{$\rho$-POMDPs}

\sloppy 
Facing the task of informative planning, we will use a model which is an extension of the well-known Partially Observable Markov Decision Process (POMDP). This extension is referred to as $\rho$-POMDP and is modeled as a tuple $\langle \mathcal{X}, \mathcal{A}, \mathcal{Z}, \bel{\X_0}, \mathbb{P}_T, \mathbb{P}_Z, \rho \rangle$, where $\mathcal{X}$ is the state space, $\mathcal{A}$ is the action space, and $\mathcal{Z}$ is the observation space; $\bel{\X_0} \bydef \prob{\X_0}$ is the prior belief over the state,  $\mathbb{P}_T$ is the probabilistic transition model, and $\mathbb{P}_Z$ is the probabilistic observation model; $\rho \left( \bel{\X_t}, a_t \right)$ is a belief-dependent immediate reward function.

%A Partially Observable Markov Decision Process (POMDP) is modeled as a tuple $\langle \mathcal{X}, \mathcal{A}, \mathcal{Z}, \bel{\X_0}, \mathbb{P}_T, \mathbb{P}_Z, r \rangle$, where $\mathcal{X}$ is the state space, $\mathcal{A}$ is the actions space, and $\mathcal{Z}$ is the observations space; $\bel{\X_0} \bydef \prob{\X_0}$ is the prior belief over the state,  $\mathbb{P}_T$ is the probabilistic transition model, and $\mathbb{P}_Z$ is the probabilistic observation model; $r \left( \X_t, a_t \right)$ is an immediate reward function. %representing the planning goals.

The prior belief and probabilistic models are used in the inference layer for determining future posterior beliefs. The belief over the state $\X_t$ at time $t$ is defined by $\bel{\X_t} \bydef \prob{\X_t \mid \his_t}$,
where $\his_t = \left\{ a_{0:t-1}, \z_{1:t} \right\}$ is the history, containing all actions $a_{0:t-1}$ and observations $\z_{1:t}$ acquired up to time $t$.
The transition model $\mathbb{P}_T \bydef \prob{x_t \mid \X_{t-1}^{tr}, a_{t-1}}$ defines the distribution of the successor state $x_t$, given a subset of its previous state $\X_{t-1}^{tr} \subseteq \X_{t-1}$ participating in the transition, and the chosen action $a_{t-1}$.
In this paper, we use the \emph{smoothing} formulation, where the successor state is \emph{augmented} to the previous, thus constructing the \emph{joint} successor state $\X_t = \left\{ \X_{t-1}, x_t \right\}$. This formulation means that the state's dimension increases in time. 
The observation model $\mathbb{P}_Z \bydef \prob{\z_t \mid \X_t^{obs}}$ defines the conditional distribution of receiving an observation $\z_t$, given a subset of the state $\X_t^{obs} \subseteq \X_t$ which participates in generating the observation.

For example, in the case of active (full) SLAM, the state is defined as the union of all poses and landmarks. The transition model can be formulated between two consecutive poses, and the observation model can be formulated such that an observation is generated given the last pose and a specific landmark. This example is illustrated in the factor graph in Figure~\ref{fig:factorgraph_involved}, where $p$ refers to poses, $l$ to landmarks and the factor nodes represent the probabilistic constraints between the variables, given with the motion and observation models.

Using Bayes' rule and the chain rule, the belief can be defined recursively as $\bel{\X_t} = \eta \FT \FZ \bel{\X_l}$,
where $\FT \triangleq \prod_{i = l+1}^{t} \prob{x_i \mid \X_{i-1}^{tr}, a_{i-1}}$ is the sequential transition model, $\FZ \triangleq \prod_{j = l+1}^{t} \prob{\z_j \mid \X_j^{obs}}$ the sequential observation model, and $\eta^{-1} \triangleq \prod_{k = l+1}^{t} \prob{\z_k \mid \his_k^{-}}$ the sequential normalizer, where $\his_k^{-} \bydef \his_k \setminus \z_k$. 

%
%\VI{[maybe better to start directly with the belief-dependent reward and then state it can be multi-objective...]} 
The tasks of the planning scheme are represented with the immediate reward function $\rho \left( \bel{\X_t}, a_t \right)$. Obviously, each planning task might involve multiple different (and sometimes contradicting) tasks, such as energy consumption and time to reach a goal, thus the reward functions might be shaped with multiple different terms. Having the reward defined as belief-dependent allows to express information-gathering tasks. %\VI{[not sure if this location makes sense - maybe better to move to the end of this section (before section 3.2 )]}

%\add{In this work, we focus on making informative planning more efficient.} The reward in our formulation must thus also express information-gathering tasks, which in turn means that the reward has to be belief-dependent. We thus use $\rho$-POMDP, an extension of POMDP, whose reward is $\rho_t \bydef \rho \left( \bel{\X_t}, a_t \right)$.

Planning $T$ steps into the future, the objective is then to find an action sequence $a_{0:T-1}$ which maximizes the expected sum of rewards, denoted as the objective function, $J \left( \bel{\X_0}, a_{0:T-1} \right) = \underset{\mathcal{Z}_{1:T}}{\mathbb{E}} \left[ \sum_{t=0}^{T-1} \rho_t + \rho_T \right]$,  where $\mathcal{Z}_{1:T}$ is the sequential space of future observations, $\rho_t \bydef \rho \left( \bel{\X_t, a_t} \right)$ is the reward at each time $t$, and $\rho_T \bydef \rho \left( \bel{\X_T} \right)$ is a terminal reward. Due to commutativity, the objective function can also be written as the sum of expected rewards, $J \left( \bel{\X_0}, a_{0:T-1} \right) = \sum_{t=0}^{T-1} \left[ \underset{\mathcal{Z}_{1:t}}{\mathbb{E}} \left[ \rho_t \right] \right] + \underset{\mathcal{Z}_{1:T}}{\mathbb{E}} \left[ \rho_T \right]$, which means that we can evaluate the expected rewards rather than the rewards themselves.

We note that although the problem is formulated as an open loop, our approach also supports a close loop formulation, in which the objective is to find a policy $\pi$ instead of an action sequence. This is since our approach focuses on evaluating the (expected) rewards in the objective function. Focusing on the objective function evaluation also means that other building blocks of the planning task, such as the inference engine and the optimization solver, can be chosen independently.


\subsection{Information-theoretic rewards}

A commonly used information-theoretic reward is negative (differential) entropy. The entropy of the state $\X_t \in \mathcal{X}_t$, distributed with $\bel{\X_t}$, is defined as
\begin{equation}
	\ent{\X_t \mid \his_t} \bydef -\int_{\mathcal{X}_t} \bel{\X_t} \log \bel{\X_t} d\X_t.
\end{equation}
%
Another commonly used information-theoretic reward is information gain (IG), which quantifies the amount of information gained for a certain variable by knowing the value of another variable. For the case where the state changes between time steps, as presented in the previous subsection, the original definition of IG is insufficient, since it does not account for the additional uncertainty obtained by changes in the state. Thus, we define the reward more generally as the difference between the entropies of the prior state $\X_0$ and the successor state $\X_t$. We remind that in our formulation the posterior state is augmented, i.e. $\X_t = \left\{ \X_0, \x_{1:t} \right\}$, thus we will refer to this reward as \emph{augmented} IG, defined at each time $t$ as
\begin{equation}
	\label{eq:augmented_ig_full}
	\igaug{\X_0}{x_{1:t}}{\Z_{1:t}=z_{1:t} \mid a_{0:t-1}}
	\bydef \ent{\X_0} - \ent{\X_t \mid \Z_{1:t}=z_{1:t},  a_{0:t-1}},
\end{equation}
where $\Z_{1:t}$ represents the observation sequence as a random variable, and the symbol $\augplus$ provides a distinction between the prior state $\X_0$ and the new, augmented subset $x_{1:t}$ of the successor state $\X_t$. This distinction is necessary since $x_{1:t}$ only appears in the posterior entropy term, while $\X_0$ appears in both terms. We then define the corresponding expected reward, \emph{augmented} mutual information (MI), as
\begin{equation}
	\label{eq:augmented_mi_full}
	\begin{aligned}
		\miaug{\X_0}{x_{1:t}}{\Z_{1:t} \mid a_{0:t-1}} 
		&\bydef \underset{\mathcal{Z}_{1:t}}{\mathbb{E}} \Big[ \igaug{\X_0}{x_{1:t}}{\Z_{1:t}=z_{1:t}, a_{0:t-1}} \Big] \\
		&= \ent{\X_0} - \ent{\X_t \mid \Z_{1:t}, a_{0:t-1}}.
	\end{aligned}
\end{equation}
We note that augmented IG and augmented MI are generalizations of the original IG and MI. The definitions of the latter are provided in Appendix \ref{sec:Info_theo}. %Section 1 in the supplementary material\footnote{https://tinyurl.com/mryt7ac8.}.

For the purposes of planning, since negative entropy and augmented IG differ only by the value $\ent{\X_0}$, which is constant for each action, using any of these as rewards is equivalent. We further continue to present our approach by choosing augmented IG as the reward, $\rho_t = \igaug{\X_0}{x_{1:t}}{\Z_{1:t}=z_{1:t} \mid a_{0:t-1}}$ (for the terminal reward as well), which dictates that the expected reward is augmented MI. The basis of our approach focuses on the evaluation of the augmented MI, thus we will present it over the augmented MI at time $t$ alone. Naturally, it will apply for the entire horizon. 

For readability, we  denote the prior state as $\X = \X_0$, the state at time $t$ as $\X' = \X_t = \left\{\X_0, x_{1:t} \right\}$ and the augmented part of the state as $\Xnew = \left\{ x_{1:t} \right\}$. Also, the future observation sequence up to time $t$ is denoted as $\Z = \left\{ \Z_{1:t} \right\}$ and its space is denoted as $\mathcal{Z} = \left\{ \mathcal{Z}_{1:t} \right\}$. Lastly, we omit the conditioning over future actions. The augmented MI  \eqref{eq:augmented_mi_full} then becomes
%
\begin{equation}
	\label{eq:mi_aug_def}
	\begin{aligned}
		\miaug{\X}{\Xnew}{\Z} \bydef \ent{\X} - \ent{\X' \mid Z} 
		 = \ent{\X} - \ent{\X, \Xnew \mid Z}.
	\end{aligned}
\end{equation}
%
The evaluation of any of the presented information-theoretic terms involves integration over the state-space, thus we might face the Curse of Dimensionality when the state is high-dimensional. When there are multiple tasks, then, arguably, evaluating the information-theoretic terms involves the heaviest calculations of the objective function. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Information-gathering tasks} \label{subsec:info_task}
%\VI{[cancel subsection, reduce drastically (move to supplementary)]\\}
%%
%We start by introducing some known information-theoretic terms for the simple case in which the state is static, i.e. $\X_t = \X$, $\forall t$. A commonly used information-theoretic reward is negative (differential) entropy. The entropy of the state $\X \in \mathcal{X}$, distributed with $\prob{X}$, is defined as
%\begin{equation}
%	\ent{\X} \bydef -\int_{\mathcal{X}} \prob{\X} \log \prob{\X} d\X.
%\end{equation}
%Getting an observation $z \in \mathcal{Z}$, without transitioning the state, yields
%\begin{equation}
%	\label{eq:ent_def}
%	\ent{\X \mid Z=z} \bydef -\int_{\mathcal{X}} \prob{\X \mid Z=z} \log \prob{\X \mid Z=z} d\X,
%\end{equation}
%%
%and the expected reward, referred to as conditional entropy, is then defined as
%\begin{equation}
%	\begin{gathered}
%		\ent{\X \mid \Z} = \underset{\mathcal{Z}}{\mathbb{E}} \Big[ \ent{\X \mid \Z=z} \Big]
%		= -\iint_{\mathcal{X}, \mathcal{Z}} \prob{\X, \Z} \log \prob{\X \mid \Z} d\X d\Z.
%	\end{gathered}
%\end{equation}
%%
%Another commonly used information-theoretic reward is information gain (IG), which quantifies the amount of information gained for a certain variable by knowing the value of another variable. It is defined as the difference between the entropy prior to this additional knowledge and the entropy afterwards
%\begin{equation}
%\ig{X}{Z=z} \bydef \ent{\X} - \ent{\X \mid \Z=z}.
%\end{equation}
%%
%
%Similarly to the entropy case, we introduce the expected reward of IG, which is referred to as the mutual information (MI).
%It can also be defined as the difference between the entropy of the state and the expected entropy of the state given the new observation
%\begin{equation}
%\begin{aligned}
%\mi{\X}{\Z}
%\bydef \underset{\mathcal{Z}}{\mathbb{E}} \Big[ \ig{X}{Z=z} \Big]
%= \ent{\X} -\ent{\X \mid \Z}.
%\end{aligned}
%\label{eq:MI}
%\end{equation}
%%
%While there are situations in which getting a specific value of $Z$ increases the uncertainty (entropy), thus making IG negative, MI on the other hand is non-negative, i.e. $\mi{\X}{\Z} \geq 0$. It means that in \emph{expectation} the variables can only add information about each other.
%
%For the case where the state changes between time steps, as presented in the previous subsection, the original definitions of IG and MI are insufficient, since these do not account for the additional uncertainty obtained by changes in the state.
%Thus, we define the reward more generally as the difference between the entropies of the prior state $\X_0$ and the successor state $\X_t$. We remind that in our formulation the posterior state is augmented, i.e. $\X_t = \left\{ \X_0, \x_{1:t} \right\}$, thus we will refer to this reward as \emph{augmented} IG, defined at each time $t$ as
%\begin{equation}
%	\label{eq:augmented_ig_full}
%	\begin{aligned}
%		\igaug{\X_0}{x_{1:t}}{\Z_{1:t}=z_{1:t} \mid a_{0:t-1}}
%		&\bydef \ent{\X_0} - \ent{\X_t \mid \Z_{1:t}=z_{1:t},  a_{0:t-1}} \\
%		&= \ent{\X_0} - \ent{\X_0, x_{1:t} \mid \Z_{1:t}=z_{1:t}, a_{0:t-1}},
%	\end{aligned}
%\end{equation}
%where the symbol $\augplus$ provides a distinction between the prior state $\X_0$ and the new, augmented subset $x_{1:t}$ of the successor state $\X_t$. 
%This distinction is necessary since $x_{1:t}$ only appears in the posterior entropy term, while $\X_0$ appears in both terms.
%The corresponding expected reward, \emph{augmented} MI, is then defined at each time $t$ as
%\begin{equation}
%	\label{eq:augmented_mi_full}
%	\begin{aligned}
%		\miaug{\X_0}{x_{1:t}}{\Z_{1:t} \mid a_{0:t-1}} 
%		&\bydef \underset{\mathcal{Z}_{1:t}}{\mathbb{E}} \Big[ \igaug{\X_0}{x_{1:t}}{\Z_{1:t}=z_{1:t}, a_{0:t-1}} \Big] \\
%		&= \ent{\X_0} - \ent{\X_t \mid \Z_{1:t}, a_{0:t-1}}.
%	\end{aligned}
%\end{equation}
%%
%Note that augmented IG and augmented MI converge to IG and MI, respectively, when there is no change in the state, i.e. $x_{1:t} = \emptyset$ and $\X_t = \X_0$. Thus, augmented IG and augmented MI can be considered as generalizations of IG and MI.
%
%For the purposes of planning, since negative entropy and augmented IG differ only by the value $\ent{\X_0}$, which is constant for each action, using any of these as rewards is equivalent. We further continue to present our approach by choosing augmented IG as the reward, $\rho_t = \igaug{\X_0}{x_{1:t}}{\Z_{1:t}=z_{1:t} \mid a_{0:t-1}}$ (for the terminal reward as well), which dictates that the expected reward is augmented MI. The basis of our approach focuses on the evaluation of the augmented MI, thus we will present it over the augmented MI at time $t$ alone. Naturally, it will apply for the entire horizon. For readability, we can then denote the prior state as $\X = \X_0$, the state at time $t$ as $\X' = \X_t = \left\{\X_0, x_{1:t} \right\}$ and the augmented part of the state as $\Xnew = \left\{ x_{1:t} \right\}$. Also, the future observations sequence up to time $t$ is denoted as $\Z = \left\{ \Z_{1:t} \right\}$ and its space is denoted as $\mathcal{Z} = \left\{ \mathcal{Z}_{1:t} \right\}$. Lastly, we omit the conditioning over future actions. The augmented MI definition \eqref{eq:augmented_mi_full} then becomes
%\begin{equation}
%	\label{eq:mi_aug_def}
%	\begin{aligned}
%		\miaug{\X}{\Xnew}{\Z} & \bydef \ent{\X} - \ent{\X' \mid Z} \\
%		& = \ent{\X} - \ent{\X, \Xnew \mid Z}.
%	\end{aligned}
%\end{equation}
%
%The evaluation of any of the presented info-theoretic terms involves integration over the state-space, thus we might face the Curse of Dimensionality when the state is high-dimensional.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Non-parametric entropy estimation} \label{subsec:nonpara_ent_est}
%Naively, for any of the above rewards and expected rewards, some variant of the entropy must be calculated. Having a belief over the state $\X \in \mathbb{R}^D$ which is non-parametric, it is usually approximated by a weighted particle set $\{ (\X^{(i)}, w^{(i)}) \}_{i=1}^{N}$ with normalized weights. Thus the entropy is approximated as well using this particle set.
% TODO: add citations for entropy estimators papers
%Several entropy estimators exist in literature, each has its own advantages and disadvantages compared to the others. Yet, the problem of state dimension stays the same for all. As it gets higher, a higher number of samples would be required. One of these estimators, as can be seen in \cite{beirlant1997nonparametric}, is the re-substitution estimator, for which the entropy is estimated as

For any of the presented information-theoretic terms, one possible calculation scheme is to go through calculation of entropy. Having  a non-parametric belief over a state $\X \in \mathbb{R}^D$, it is usually approximated by a weighted particle set $\{ (\X^{(i)}, w^{(i)}) \}_{i=1}^{N}$ with normalized weights, where $\X^{(i)}$ is the $i$-th particle, $w^{(i)}$ is the weight of the $i$-th particle, and $N$ is the number of particles. The Curse of Dimensionality in this case means that in order to have sufficient resolution to represent the belief, the number of particles $N$ needs to be exponential in the dimension $D$, i.e. $N \propto \alpha^D$ where $\alpha \geq 1$. The entropy in this case is approximated as well using this particle set, and thus will suffer from the Curse of Dimensionality as well, as will further be shown. 
Several entropy estimators exist in literature, each has its own advantages and disadvantages. The most well-known estimators can be found in \cite{Beirlant97jmss}. One of these estimators, for example, is the re-substitution estimator, for which the entropy is estimated as $\hat{\mathcal{H}} \left[ \X \right] \bydef \sum_{i=1}^{N} w^{(i)} \log \hat{b} \left[ \X^{(i)} \right]$,
where $\hat{b} \left[ \X \right]$ is an approximation of the belief obtained by a probability distribution estimator such as Kernel Density Estimator (KDE). The computational complexity of calculating entropy with the re-substitution estimator with KDE is $O \left( N^2 D \right)$.
Another estimator, presented in \cite{Stowell09spl}, performs $k$-d partitioning of the state-space, and thus achieves a complexity of $O \left( N \log N \right)$. There are many more estimators, such as estimators which are based on nearest-neighbor or $m_n$-spacings, however analyzing these is outside the scope of this work.
%\VI{we do not here analyze these [suggest to rephrase - analyzing these is outside the scope of this work]}.\VI{[if there is a survey/review paper on these estimators, you can refer to it here]}

Although the complexity of the presented estimators might not seem to have an exponential relation to the state's dimension $D$, or any relation at all, we remind that $N$ should be exponential with $D$ in order to get an accurate enough estimation, thus the complexity of any estimator is exponential with the dimension $D$, even if not explicitly.

%Due to curse of dimensionality, in order to have sufficient resolution to represent the belief, the number of samples should be exponential with the dimension, making the complexity exponential with the dimension as well.
% TODO: mention this is only the complexity of the reward itself, yet without expectation over future observations

==> 2022 Arxiv/04-Approach.tex <==
%\usetikzlibrary{fadings}
%\usetikzlibrary{patterns}
%\usetikzlibrary{shadows.blur}
%\usetikzlibrary{shapes}

\graphicspath{ {./Figures/}}

Our work includes multiple contributions when approaching the problem of informative planning with high-dimensional non-parametric beliefs. These will be presented in different sections.
Our first contribution is an exact mathematical derivation which shows that the dimension of the belief-space can be reduced for the calculation of augmented MI by only exploiting the structure of the problem, which is true as well for the case of the original definition of MI. It thus provides a solution to the curse of dimensionality. We refer to this part of the approach as \invmi{}.
As our second contribution, we derive a method that allows to avoid the explicit reconstruction of the beliefs' surfaces usually required for the augmented MI calculation. We then use this to construct an estimator, which we refer to as \mismc{}.
In the last section, we discuss how \invmi{} and \mismc{} can be used together with existing solvers of the informative planning problem, more specifically tree-based solvers.

\subsection{Dimensionality reduction for MI calculation} \label{sec:dim_red}

We aim at reducing the complexity of calculating the augmented MI over a high-dimensional state $\X \in \mathbb{R}^D$, where $D \gg 1$, distributed with a non-parametric belief.
As the dimension increases, the number of samples required to get the same accuracy, and thus the complexity, exponentially increases.

More specifically, the \emph{key idea} of our approach is to reduce the dimensionality of the problem by exploiting its \emph{structure}. As in the works \cite{Kopitkov17ijrr}, \cite{Elimelech17icra}, it starts by dividing the high-dimensional \emph{prior} state into two subsets, such that $\X = \left\{ \Xinv, \Xnot \right\}$.
We remind that only subsets of the state participate in the probabilistic transition and observation models, $\mathbb{P}_T$ and $\mathbb{P}_Z$, respectively.
The same also applies for the sequential counterparts, $\FT$ and $\FZ$, defined earlier. Thus, $\Xinv \in \mathbb{R}^d$, which we will refer to as the \emph{involved} subset of the state, is defined as a union of all variables in the prior state $\X = \X_0 $ which participate in generating future state transitions and future observations
%
\begin{equation}
	\label{eq:inv_def}
	\Xinv = \left[ \bigcup_{i=1}^{t} \Big[ \X_{i-1}^{tr} \cup \X_{i}^{obs} \Big] \right] \cap \X,
\end{equation}
%
where the intersection with the prior state $\X$ is to emphasize that while the subsets $\X_{i-1}^{tr}$ and $\X_{i}^{obs}$ might also include new augmented variables $\Xnew$, which are inherently involved, we define $\Xinv$ as a subset of the prior alone.

Furthermore, this subset is usually very small compared to the dimension of the entire state, i.e. $d \ll D$, a fact which is of key importance in our approach.
Determining the involved subset is done heuristically, as is naturally done when transitioning and generating future measurements.
This idea is also illustrated with a SLAM example in Figure~\ref{fig:illustration_involved}. In this example, the involved variables are the prior pose and observed landmarks.

More generally, we define $\Xinvp$, a subset \emph{containing} the involved rather \emph{only} the involved, such that $\Xinv \subseteq \Xinvp \subseteq \X$. This subset has larger dimensions, yet it might still be much smaller in dimensions compared to the entire state. When referring to the involved variables, we also refer to this subset.

%\subsubsection*{Phase 1: MI}
%%
%We will start by analyzing a degenerate problem, for which the state $\Xtild$ is static or already transitioned, and we only wish to quantify the expected amount of information the future observations $\Ztild$ will add. We then define $\Xinvt$ as just the union of all variables in the state which participate in generating future observations. In this case, we get back to the original MI definition in eq.~(\ref{eq:MI}).
%%
%\begin{theorem}
%		\label{th:mi_involved}
%		Let \(\Xtild\) be some state and \(\Ztild\) be an observation sequence over a subset of this state, \(\tilde{\X}^{in} \subseteq \Xtild\), such that the observation model is \( \prob{\Ztild \mid \Xtild} \equiv \prob{\Ztild \mid \Xinvt} \). Then,
%		\begin{equation}
%			\mi{\tilde{\X}}{\tilde{\Z}} = \mi{\tilde{\X}^{in}}{\tilde{\Z}}.
%		\end{equation}
%\end{theorem}
%%
%The proof of this theorem, as well as the following theorems, lemmas and propositions, is given in the appendix.
%
%In words, Theorem~\ref{th:mi_involved} states that the information the observations entail over the state is exactly the information they entail over the involved variables alone. This, in turn, means that in order to get an \emph{exact} solution, it is sufficient to solve a much lower dimensional problem. A simple example to illustrate this, is when an autonomous robot needs to choose between observing two landmarks, one with low prior marginal uncertainty and one with a higher uncertainty. Theorem~\ref{th:mi_involved} suggests that it would definitely be more beneficial to observe the more uncertain one, regardless of the correlations (which are already taken into account in the marginalization process).
%
%This conclusion is very similar to the one in \cite{Kopitkov17ijrr}, yet a bit different. While the conclusion there seems more general in the sense that it is true for the reward itself without expectation (IG), it is only valid for the Gaussian case. Note in our approach we do not assume any specific distribution.
%Although the most general motivation is to reduce the complexity of calculating the reward alone (IG), unfortunately, to this end, we were unable to extend our approach to support that, which is the reason we directly calculate the expected reward. We suspect that this extension is only possible for uni-modal distributions, but this assumption dictates that it is not a generalization, but rather a compromise between the ability to plan for any distribution and the ability to efficiently calculate the reward alone. While going in this direction might still be more general than \cite{Kopitkov17ijrr}, we leave this idea for future research.
%Going further in this paper, we will also show that for $\rho$-POMDP this issue is immaterial.

%\emph{Remark:} We would like to note that \cite{Chli09thesis}, for the more specific case of feature selection, has come to an analogous conclusion. In that work, the variables were features. The probability distribution was then approximated as a tree, in which the nodes are the features and the vertices are dependencies between these features. Then, the authors concluded that the MI a node in this tree is predicted to provide to the rest of the nodes in this tree is equivalent to the MI it is predicted to give to its neighbors alone. This conclusion can of course be generalized to any tree. Our problem can be formulated as well as a tree, in which the nodes are $\Xnott$, $\Xinvt$ and $\Ztild$, since there is no dependence between $\Xnott$ and $\Ztild$, thus we could have used the above conclusion to prove Theorem~\ref{th:mi_involved}.
%The works \cite{julian2014mutual} and \cite{zhang2020fsmi} has also come to an analogous conclusion, yet again the context of these works, active mapping, is very specific.
%We also note none of these works deal with the more general case of augmentation, which we discuss next.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Continuing with our initial problem formulation, in which the state is transitioned (augmented, more specifically) and we wish to also take into account the uncertainty this transitioning has introduced, 
With the augmented MI definition in eq.~(\ref{eq:mi_aug_def}) we derive the following Lemma,

%
\begin{lem}
	\label{le:mi_miaug_relation}
	Let \(\X\) be some prior state, and \(\X' = \left\{ \X, \Xnew \right\}\) be a successor state, where \(\Xnew\) is the augmented subset of the successor state. Let the multivariate random variable \(\Z\) denote an observation sequence over this successor state. Then, the relation between MI and augmented MI is
	\begin{equation}
		\miaug{\X}{\Xnew}{\Z} = \mi{\X, \Xnew}{\Z} - \ent{\Xnew \mid \X}.
	\end{equation}
\end{lem}
%
where $\mi{\X, \Xnew}{\Z} \bydef \ent{\X, \Xnew} - \ent{\X, \Xnew \mid \Z}$ is the definition of the original MI over the joint state $\left\{ \X, \Xnew \right\}$.
The proof of this lemma, as well as the following theorems, lemmas and propositions, is given in Appendices \ref{sec:invmi} and \ref{sec:mismc}. 
In words, the difference between the two MI variants is the expected uncertainty obtained directly from transitioning the state.
%Note that while MI is non-negative, augmented MI on the other hand can be negative because of the additional term.
Using this Lemma, we  derive the following Theorem,
%
\begin{theorem}
	\label{th:mi_aug_involved}
	Let \(\X\) be some prior state, and \(\X' = \left\{ \X, \Xnew \right\}\) be a successor state, where \(\Xnew\) is the augmented subset of the successor state. Let the multivariate random variable \(\Z\) be an observations sequence over a subset of the successor state, \( \left\{\Xinvp, \Xnew \right\} \subseteq \X'\), such that \( \prob{\Z \mid \X, \Xnew} \equiv \prob{\Z \mid \Xinvp, \Xnew} \). Then,
	\begin{equation}
		\miaug{\X}{\Xnew}{\Z} = \miaug{\Xinvp}{\Xnew}{\Z}.
	\end{equation}
\end{theorem}
%
%Meaning that the same conclusion we have got for the unaugmented case applies also for the case of augmentation.
In words, Theorem~\ref{th:mi_aug_involved} states that the expected information to be gained about the entire state between these time steps is exactly the expected information to be gained about the involved variables $\Xinvp$ alone. This, in turn, means that in order to get an \emph{exact} solution, it is sufficient to solve a much lower dimensional problem. We note that this is regardless of the correlations, which are already taken into account in the marginalization process.

The subset $\Xinv$ depends on the specific action and its observations, such that if we have $n$ candidate actions, each action might have different involved variables. We will denote the involved subset for the $j$-th action as $\Xinvi{j}$. Reasoning about the exact involved variables and marginalizing out the uninvolved variables for each action might be costly operations which will eventually make this whole approach worthless. When using the more general definition of the involved variables, $\Xinvp$, it allows choosing $\Xinvp = \Xinvi{1} \cup \Xinvi{2} \cup \dots \cup \Xinvi{n}$, which results in a one-time marginalization rather than marginalizing for each action separately. This concept is similar to the one suggested in \cite{Kopitkov17ijrr}. Moreover, using $\Xinvp$ might be helpful in cases we have an easy way to calculate marginalized beliefs of subsets which are not exactly the involved but contain them. Despite all this, for readability reasons we will continue to refer to the involved variables as $\Xinv$ rather than $\Xinvp$, yet we emphasize that the following is true for $\Xinvp$ as well.

The result of Theorem~\ref{th:mi_aug_involved} is also illustrated as an information diagram in Figure~\ref{fig:augmented_info_diag}. Note that discarding (marginalizing out) the subset $\Xnot \bydef \X \setminus \Xinv$ (blue circle) does not affect the calculation since the shaded areas we are calculating remain the same.

While this conclusion might remind the one in \cite{Kopitkov17ijrr}, which considered only the Gaussian case, it can be viewed as a non-trivial extension to an arbitrary distribution. Specifically, Theorem~\ref{th:mi_aug_involved} states that \emph{in expectation} the augmented IG and its involved counterpart are exactly equal, no matter how the belief is distributed.


%% Pattern Info
%\tikzset{
%	pattern size/.store in=\mcSize, 
%	pattern size = 5pt,
%	pattern thickness/.store in=\mcThickness, 
%	pattern thickness = 0.3pt,
%	pattern radius/.store in=\mcRadius, 
%	pattern radius = 1pt}
%\makeatletter
%\pgfutil@ifundefined{pgf@pattern@name@_h3dylt67w}{
%	\pgfdeclarepatternformonly[\mcThickness,\mcSize]{_h3dylt67w}
%	{\pgfqpoint{0pt}{-\mcThickness}}
%	{\pgfpoint{\mcSize}{\mcSize}}
%	{\pgfpoint{\mcSize}{\mcSize}}
%	{
%		\pgfsetcolor{\tikz@pattern@color}
%		\pgfsetlinewidth{\mcThickness}
%		\pgfpathmoveto{\pgfqpoint{0pt}{\mcSize}}
%		\pgfpathlineto{\pgfpoint{\mcSize+\mcThickness}{-\mcThickness}}
%		\pgfusepath{stroke}
%}}
%\makeatother
%\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

%This conclusion is very similar to the one in \cite{Kopitkov17ijrr}, yet a bit different. While the conclusion there seems more general in the sense that it is true for the reward itself without expectation (IG), it is only valid for the Gaussian case. Note in our approach we do not assume any specific distribution.
%\VI{Although the most general motivation is to reduce the complexity of calculating the reward alone (IG), unfortunately, to this end, we were unable to extend our approach to support that, which is the reason we directly calculate the expected reward. [rephrase]} Going further in this paper, we will also show that for $\rho$-POMDP this is immaterial.


% Information diagram
%\begin{figure}
%	\centering
%%	\scalebox{0.45}{
%%		\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%%			%uncomment if require: \path (0,441); %set diagram left start at 0, and has height of 441
%%			
%%			%Curve Lines [id:da4033650573064922] 
%%			\draw [draw opacity=0][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.75] [line join = round][line cap = round]   (165.5,189.8) .. controls (165.5,183.8) and (170.62,183.12) .. (173.5,178.8) .. controls (175.01,176.54) and (174.83,173.46) .. (175.5,170.8) .. controls (176.2,167.99) and (183.3,162.47) .. (185.5,158.8) .. controls (192.5,150.8) and (197.5,147.8) .. (206.5,141.8) .. controls (211.5,137.8) and (223.4,132.98) .. (230.5,131.8) .. controls (239.5,126.8) and (247.15,128.67) .. (256.5,126.8) .. controls (266.92,124.72) and (284.5,127.8) .. (296.5,129.8) .. controls (298.26,130.68) and (285.99,133.68) .. (285.5,133.8) .. controls (282.28,134.61) and (278.83,136.93) .. (274.5,137.8) .. controls (265.5,143.8) and (256.28,154.02) .. (251.5,158.8) .. controls (248.48,161.82) and (243.87,163.25) .. (241.5,166.8) .. controls (240.1,168.9) and (240.79,173.51) .. (238.5,175.8) .. controls (231.12,183.18) and (225.8,204.07) .. (224.5,215.8) .. controls (223.33,226.37) and (223.5,237.8) .. (223.5,249.8) .. controls (223,251.53) and (218.13,245.9) .. (217.5,245.8) .. controls (209.8,244.52) and (205.71,239.06) .. (198.5,236.66) .. controls (192.5,229.8) and (191.52,227.82) .. (186.5,222.8) .. controls (178.18,214.48) and (173.85,209.85) .. (169.5,196.8) .. controls (168.22,192.95) and (164.5,192.46) .. (164.5,186.8) ;
%%			%Curve Lines [id:da9329263652587878] 
%%			\draw [draw opacity=0][pattern=_h3dylt67w,pattern size=6pt,pattern thickness=1.5pt,pattern radius=0pt, pattern color={rgb, 255:red, 0; green, 0; blue, 0}][line width=0.75] [line join = round][line cap = round]   (165.5,189.8) .. controls (165.5,183.8) and (170.62,183.12) .. (173.5,178.8) .. controls (175.01,176.54) and (174.83,173.46) .. (175.5,170.8) .. controls (176.2,167.99) and (183.3,162.47) .. (185.5,158.8) .. controls (192.5,150.8) and (197.5,147.8) .. (206.5,141.8) .. controls (211.5,137.8) and (223.4,132.98) .. (230.5,131.8) .. controls (239.5,126.8) and (247.15,128.67) .. (256.5,126.8) .. controls (266.92,124.72) and (284.5,127.8) .. (296.5,129.8) .. controls (298.26,130.68) and (285.99,133.68) .. (285.5,133.8) .. controls (282.28,134.61) and (278.83,136.93) .. (274.5,137.8) .. controls (265.5,143.8) and (256.28,154.02) .. (251.5,158.8) .. controls (248.48,161.82) and (243.87,163.25) .. (241.5,166.8) .. controls (240.1,168.9) and (240.79,173.51) .. (238.5,175.8) .. controls (231.12,183.18) and (225.8,204.07) .. (224.5,215.8) .. controls (223.33,226.37) and (223.5,237.8) .. (223.5,249.8) .. controls (223,251.53) and (218.13,245.9) .. (217.5,245.8) .. controls (209.8,244.52) and (205.71,239.06) .. (198.5,236.66) .. controls (192.5,229.8) and (191.52,227.82) .. (186.5,222.8) .. controls (178.18,214.48) and (173.85,209.85) .. (169.5,196.8) .. controls (168.22,192.95) and (164.5,192.46) .. (164.5,186.8) ;
%%			%Curve Lines [id:da4421168531852726] 
%%			\draw [draw opacity=0][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.75] [line join = round][line cap = round]   (166.5,193.66) .. controls (166.83,196.66) and (166.85,199.71) .. (167.5,202.66) .. controls (167.78,203.91) and (172.66,206.82) .. (174.5,208.66) .. controls (182.11,216.27) and (189.77,227.93) .. (198.5,236.66) .. controls (201.25,239.4) and (208.99,239.15) .. (211.5,241.66) .. controls (213.1,243.26) and (216.76,246.92) .. (218.5,248.66) .. controls (219.81,249.96) and (226.3,251.66) .. (226.5,252.66) .. controls (227.16,255.94) and (224.3,259.53) .. (225.5,262.66) .. controls (228.67,270.89) and (229.7,267.92) .. (233.7,275.92) .. controls (236.41,278.63) and (240.7,286.92) .. (237.5,281.66) .. controls (238.52,285.74) and (243.65,289.81) .. (246.5,292.66) .. controls (247.92,294.08) and (242.9,291.18) .. (250.7,296.92) .. controls (253.9,302.18) and (253.13,300.92) .. (254.5,303.66) .. controls (256.61,307.87) and (263.33,314.57) .. (269.5,317.66) .. controls (271.68,318.75) and (276.43,321.52) .. (277.5,321.66) .. controls (280.17,321.99) and (283.6,320.76) .. (285.5,322.66) .. controls (286.33,323.48) and (292.54,324.6) .. (291.5,324.66) .. controls (276.98,325.51) and (277.67,326.04) .. (265.79,327.12) .. controls (261.36,327.53) and (256.16,329.82) .. (251.5,328.66) .. controls (250.78,328.48) and (251.22,326.84) .. (250.5,326.66) .. controls (244.63,325.19) and (236,325.39) .. (230.5,324.66) .. controls (228.4,324.38) and (225.75,320.59) .. (222.5,319.66) .. controls (219.47,318.79) and (216.34,319.79) .. (213.5,318.66) .. controls (202.64,314.31) and (192.39,303.54) .. (183.5,294.66) .. controls (179.27,290.43) and (176,288.55) .. (173.79,284.12) .. controls (175.07,282.59) and (169.96,274.03) .. (168.5,269.66) .. controls (168.05,268.31) and (165.84,268.03) .. (165.5,266.66) .. controls (163.69,259.43) and (164.06,254.46) .. (162.5,246.66) .. controls (161.82,243.25) and (158.71,241.56) .. (158.5,238.66) .. controls (157.86,229.74) and (160.82,218.76) .. (161.5,212.66) .. controls (162.14,206.93) and (161.5,201.65) .. (163.5,197.66) .. controls (163.97,196.71) and (164.5,193.6) .. (164.5,194.66) .. controls (164.5,195.4) and (164.75,196.66) .. (165.5,196.66) ;
%%			%Curve Lines [id:da2780428942483901] 
%%			\draw [draw opacity=0][fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.75] [line join = round][line cap = round]   (294.1,129.34) .. controls (312.34,123.26) and (330.69,124.24) .. (347.1,128.34) .. controls (352.21,129.62) and (356.9,129.29) .. (361.1,130.34) .. controls (361.82,130.52) and (363.05,130.59) .. (363.1,131.34) .. controls (363.46,136.41) and (362.53,152.79) .. (362.1,158.34) .. controls (361.59,164.99) and (361.45,171.67) .. (361.1,178.34) .. controls (360.86,182.85) and (354.23,187.83) .. (353.1,192.34) .. controls (350.52,202.65) and (341.1,214.34) .. (334.1,225.34) .. controls (326.67,229.05) and (319.98,240.12) .. (311.1,242.34) .. controls (307.41,243.26) and (299.1,249.34) .. (295.1,248.34) .. controls (291.28,250.25) and (283.93,252.42) .. (280.1,254.34) .. controls (268.84,259.97) and (247.45,253.71) .. (235.1,252.34) .. controls (234.15,252.23) and (229.29,248.7) .. (227.1,248.34) .. controls (226.16,248.18) and (221.58,251.23) .. (221.1,248.34) .. controls (221.1,233.34) and (219.81,241.06) .. (220.1,237.34) .. controls (221.05,225.01) and (222.76,214.04) .. (225.1,202.34) .. controls (226.4,195.83) and (229.71,191.12) .. (233.1,184.34) .. controls (234.39,181.75) and (234.1,177.93) .. (235.1,175.34) .. controls (238.46,166.61) and (244.19,161.28) .. (250.1,157.34) .. controls (256.1,153.34) and (265.94,145.5) .. (270.1,141.34) .. controls (274.11,137.33) and (292.99,128.34) .. (299.1,128.34) ;
%%			%Shape: Ellipse [id:dp604915699384222] 
%%			\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=4.5]  (310.9,292.95) .. controls (276.21,249.36) and (284.05,185.4) .. (328.42,150.1) .. controls (372.79,114.79) and (436.87,121.51) .. (471.56,165.11) .. controls (506.25,208.7) and (498.41,272.66) .. (454.04,307.97) .. controls (409.67,343.27) and (345.59,336.55) .. (310.9,292.95) -- cycle ;
%%			%Shape: Ellipse [id:dp14907252596438347] 
%%			\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=4.5]  (243.44,291.46) .. controls (208.75,247.87) and (216.59,183.91) .. (260.96,148.6) .. controls (305.33,113.3) and (369.41,120.02) .. (404.1,163.62) .. controls (438.79,207.21) and (430.95,271.17) .. (386.58,306.47) .. controls (342.21,341.78) and (278.13,335.06) .. (243.44,291.46) -- cycle ;
%%			%Shape: Brace [id:dp22614282606535463] 
%%			\draw   (171.24,380.67) .. controls (171.24,385.34) and (173.57,387.67) .. (178.24,387.67) -- (320.61,387.67) .. controls (327.28,387.67) and (330.61,390) .. (330.61,394.67) .. controls (330.61,390) and (333.94,387.67) .. (340.61,387.67)(337.61,387.67) -- (482.97,387.67) .. controls (487.64,387.67) and (489.97,385.34) .. (489.97,380.67) ;
%%			%Shape: Ellipse [id:dp8015781431346674] 
%%			\draw  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=4.5]  (180.44,291.46) .. controls (145.75,247.87) and (153.59,183.91) .. (197.96,148.6) .. controls (242.33,113.3) and (306.41,120.02) .. (341.1,163.62) .. controls (375.79,207.21) and (367.95,271.17) .. (323.58,306.47) .. controls (279.21,341.78) and (215.13,335.06) .. (180.44,291.46) -- cycle ;
%%			%Shape: Ellipse [id:dp2165364938533929] 
%%			\draw  [color={rgb, 255:red, 248; green, 231; blue, 28 }  ,draw opacity=1 ][line width=4.5]  (180.63,218.53) .. controls (145.94,174.93) and (153.78,110.97) .. (198.15,75.67) .. controls (242.52,40.36) and (306.6,47.09) .. (341.29,90.68) .. controls (375.98,134.27) and (368.14,198.23) .. (323.77,233.54) .. controls (279.4,268.84) and (215.32,262.12) .. (180.63,218.53) -- cycle ;
%%			%Curve Lines [id:da8868483261943054] 
%%			\draw [line width=2.25]    (278.79,197.27) .. controls (272.1,174.6) and (222.1,142.6) .. (193.1,176.6) .. controls (164.97,209.58) and (133.08,198.34) .. (109.28,154.74) ;
%%			\draw [shift={(107.1,150.6)}, rotate = 422.95] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%%			%Curve Lines [id:da8485677356785608] 
%%			\draw [line width=2.25]    (212.79,287.12) .. controls (201.79,255.12) and (170.1,248.6) .. (141.1,282.6) .. controls (112.68,315.92) and (82.04,249.86) .. (51.65,306.5) ;
%%			\draw [shift={(49.79,310.12)}, rotate = 296.2] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%%			%Curve Lines [id:da23185241288128777] 
%%			\draw [line width=2.25]    (210.1,212.45) .. controls (171.1,227.45) and (170.1,248.6) .. (141.1,282.6) ;
%%			%Curve Lines [id:da058373919020516585] 
%%			\draw [line width=2.25]    (219.1,197.65) .. controls (201.1,181.65) and (196.1,189.65) .. (164.5,194.66) ;
%%			
%%			% Text Node
%%			\draw (169.5,39.99) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 248; green, 231; blue, 28 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{28.95pt}\setlength\topsep{0pt}
%%					\begin{center}
%%						$\displaystyle \ent{\Z}$
%%					\end{center}
%%					
%%			\end{minipage}};
%%			%% Text Node
%%			\draw (32,125.2) node [anchor=north west][inner sep=0.75pt]   [align=left] {
%%				\textcolor[rgb]{0.29,0.29,0.29}{
%%					$\begin{aligned}
%%						\mi{\Xinv, \Xnew}{Z}
%%					\end{aligned}$}};
%%			%% Text Node
%%			\draw (3,314.2) node [anchor=north west][inner sep=0.75pt]   [align=left] {
%%				\textcolor[rgb]{0.61,0.61,0.61}{
%%					$\begin{aligned}
%%						\ent{\Xnew \mid \X} = \\ 
%%						\ent{\Xnew \mid \Xinv}
%%					\end{aligned}$}};
%%			% Text Node
%%			\draw (384.5,344.22) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ] [align=left] {$\displaystyle \ent{\Xnot}$};
%%			% Text Node
%%			\draw (293.5,345.22) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle \ent{\Xinv}$};
%%			% Text Node
%%			\draw (307.23,404.23) node [anchor=north west][inner sep=0.75pt]  [rotate=-0.71] [align=left] {$\displaystyle \ent{\X, \Xnew}$};
%%			% Text Node
%%			\draw (209.5,346.22) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,opacity=1 ] [align=left] {$\displaystyle \ent{\Xnew}$};
%%	\end{tikzpicture}
%%	}
%	\scalebox{0.45}{
%	\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%		%uncomment if require: \path (0,441); %set diagram left start at 0, and has height of 441
%		
%		%Curve Lines [id:da7303946332994704] 
%		\draw [draw opacity=0][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.75] [line join = round][line cap = round]   (170.5,177.8) .. controls (170.5,171.8) and (175.62,171.12) .. (178.5,166.8) .. controls (180.01,164.54) and (179.83,161.46) .. (180.5,158.8) .. controls (181.2,155.99) and (188.3,150.47) .. (190.5,146.8) .. controls (197.5,138.8) and (202.5,135.8) .. (211.5,129.8) .. controls (216.5,125.8) and (228.4,120.98) .. (235.5,119.8) .. controls (244.5,114.8) and (252.15,116.67) .. (261.5,114.8) .. controls (271.92,112.72) and (289.5,115.8) .. (301.5,117.8) .. controls (303.26,118.68) and (290.99,121.68) .. (290.5,121.8) .. controls (287.28,122.61) and (283.83,124.93) .. (279.5,125.8) .. controls (270.5,131.8) and (261.28,142.02) .. (256.5,146.8) .. controls (253.48,149.82) and (248.87,151.25) .. (246.5,154.8) .. controls (245.1,156.9) and (245.79,161.51) .. (243.5,163.8) .. controls (236.12,171.18) and (230.8,192.07) .. (229.5,203.8) .. controls (228.33,214.37) and (228.5,225.8) .. (228.5,237.8) .. controls (228,239.53) and (223.13,233.9) .. (222.5,233.8) .. controls (214.8,232.52) and (210.71,227.06) .. (203.5,224.66) .. controls (197.5,217.8) and (196.52,215.82) .. (191.5,210.8) .. controls (183.18,202.48) and (178.85,197.85) .. (174.5,184.8) .. controls (173.22,180.95) and (169.5,180.46) .. (169.5,174.8) ;
%		%Curve Lines [id:da6348203178334813] 
%		\draw [draw opacity=0][fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.75] [line join = round][line cap = round]   (170.5,177.8) .. controls (170.5,171.8) and (175.62,171.12) .. (178.5,166.8) .. controls (180.01,164.54) and (179.83,161.46) .. (180.5,158.8) .. controls (181.2,155.99) and (188.3,150.47) .. (190.5,146.8) .. controls (197.5,138.8) and (202.5,135.8) .. (211.5,129.8) .. controls (216.5,125.8) and (228.4,120.98) .. (235.5,119.8) .. controls (244.5,114.8) and (252.15,116.67) .. (261.5,114.8) .. controls (271.92,112.72) and (289.5,115.8) .. (301.5,117.8) .. controls (303.26,118.68) and (290.99,121.68) .. (290.5,121.8) .. controls (287.28,122.61) and (283.83,124.93) .. (279.5,125.8) .. controls (270.5,131.8) and (261.28,142.02) .. (256.5,146.8) .. controls (253.48,149.82) and (248.87,151.25) .. (246.5,154.8) .. controls (245.1,156.9) and (245.79,161.51) .. (243.5,163.8) .. controls (236.12,171.18) and (230.8,192.07) .. (229.5,203.8) .. controls (228.33,214.37) and (228.5,225.8) .. (228.5,237.8) .. controls (228,239.53) and (223.13,233.9) .. (222.5,233.8) .. controls (214.8,232.52) and (210.71,227.06) .. (203.5,224.66) .. controls (197.5,217.8) and (196.52,215.82) .. (191.5,210.8) .. controls (183.18,202.48) and (178.85,197.85) .. (174.5,184.8) .. controls (173.22,180.95) and (169.5,180.46) .. (169.5,174.8) ;
%		%Curve Lines [id:da029992581260934736] 
%		\draw [draw opacity=0][fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.75] [line join = round][line cap = round]   (299.1,117.34) .. controls (317.34,111.26) and (335.69,112.24) .. (352.1,116.34) .. controls (357.21,117.62) and (361.9,117.29) .. (366.1,118.34) .. controls (366.82,118.52) and (368.05,118.59) .. (368.1,119.34) .. controls (368.46,124.41) and (367.53,140.79) .. (367.1,146.34) .. controls (366.59,152.99) and (366.45,159.67) .. (366.1,166.34) .. controls (365.86,170.85) and (359.23,175.83) .. (358.1,180.34) .. controls (355.52,190.65) and (346.1,202.34) .. (339.1,213.34) .. controls (331.67,217.05) and (324.98,228.12) .. (316.1,230.34) .. controls (312.41,231.26) and (304.1,237.34) .. (300.1,236.34) .. controls (296.28,238.25) and (288.93,240.42) .. (285.1,242.34) .. controls (273.84,247.97) and (252.45,241.71) .. (240.1,240.34) .. controls (239.15,240.23) and (234.29,236.7) .. (232.1,236.34) .. controls (231.16,236.18) and (226.58,239.23) .. (226.1,236.34) .. controls (226.1,221.34) and (224.81,229.06) .. (225.1,225.34) .. controls (226.05,213.01) and (227.76,202.04) .. (230.1,190.34) .. controls (231.4,183.83) and (234.71,179.12) .. (238.1,172.34) .. controls (239.39,169.75) and (239.1,165.93) .. (240.1,163.34) .. controls (243.46,154.61) and (249.19,149.28) .. (255.1,145.34) .. controls (261.1,141.34) and (270.94,133.5) .. (275.1,129.34) .. controls (279.11,125.33) and (297.99,116.34) .. (304.1,116.34) ;
%		%Shape: Ellipse [id:dp7216986376171206] 
%		\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=4.5]  (315.9,280.95) .. controls (281.21,237.36) and (289.05,173.4) .. (333.42,138.1) .. controls (377.79,102.79) and (441.87,109.51) .. (476.56,153.11) .. controls (511.25,196.7) and (503.41,260.66) .. (459.04,295.97) .. controls (414.67,331.27) and (350.59,324.55) .. (315.9,280.95) -- cycle ;
%		%Shape: Ellipse [id:dp6654621461480044] 
%		\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=4.5]  (248.44,279.46) .. controls (213.75,235.87) and (221.59,171.91) .. (265.96,136.6) .. controls (310.33,101.3) and (374.41,108.02) .. (409.1,151.62) .. controls (443.79,195.21) and (435.95,259.17) .. (391.58,294.47) .. controls (347.21,329.78) and (283.13,323.06) .. (248.44,279.46) -- cycle ;
%		%Shape: Brace [id:dp4514254783463256] 
%		\draw  [line width=1.5]  (151.5,368.67) .. controls (151.5,373.34) and (153.83,375.67) .. (158.5,375.67) -- (315.5,375.67) .. controls (322.17,375.67) and (325.5,378) .. (325.5,382.67) .. controls (325.5,378) and (328.83,375.67) .. (335.5,375.67)(332.5,375.67) -- (492.5,375.67) .. controls (497.17,375.67) and (499.5,373.34) .. (499.5,368.67) ;
%		%Shape: Ellipse [id:dp02031420030112696] 
%		\draw  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=4.5]  (185.44,279.46) .. controls (150.75,235.87) and (158.59,171.91) .. (202.96,136.6) .. controls (247.33,101.3) and (311.41,108.02) .. (346.1,151.62) .. controls (380.79,195.21) and (372.95,259.17) .. (328.58,294.47) .. controls (284.21,329.78) and (220.13,323.06) .. (185.44,279.46) -- cycle ;
%		%Shape: Ellipse [id:dp09202377552939045] 
%		\draw  [color={rgb, 255:red, 248; green, 231; blue, 28 }  ,draw opacity=1 ][line width=4.5]  (185.63,206.53) .. controls (150.94,162.93) and (158.78,98.97) .. (203.15,63.67) .. controls (247.52,28.36) and (311.6,35.09) .. (346.29,78.68) .. controls (380.98,122.27) and (373.14,186.23) .. (328.77,221.54) .. controls (284.4,256.84) and (220.32,250.12) .. (185.63,206.53) -- cycle ;
%		%Curve Lines [id:da582701427922824] 
%		\draw [line width=2.25]    (254.5,174.42) .. controls (282.5,168.42) and (293.5,134.42) .. (307.5,107.42) .. controls (321.01,81.37) and (330.8,59.97) .. (372.8,54.91) ;
%		\draw [shift={(377.5,54.42)}, rotate = 175.03] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%		
%		% Text Node
%		\draw (122.5,29.99) node [anchor=north west][inner sep=0.75pt]  [font=\LARGE,color={rgb, 255:red, 248; green, 231; blue, 28 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{48.09pt}\setlength\topsep{0pt}
%				\begin{center}
%					$\displaystyle \ent{\Z}$
%				\end{center}
%				
%		\end{minipage}};
%		% Text Node
%		\draw (386,22.2) node [anchor=north west][inner sep=0.75pt]  [font=\LARGE] [align=left] {
%			\textcolor[rgb]{0.29,0.29,0.29}{
%				$\begin{aligned}
%					\mi{\Xinv, \Xnew}{Z}
%				\end{aligned}$}};
%		% Text Node
%		\draw (386.5,323.22) node [anchor=north west][inner sep=0.75pt]  [font=\LARGE,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle \ent{\Xnot}$};
%		% Text Node
%		\draw (276.5,328.22) node [anchor=north west][inner sep=0.75pt]  [font=\LARGE,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ] [align=left] {$\displaystyle \ent{\Xinv}$};
%		% Text Node
%		\draw (288.23,387.23) node [anchor=north west][inner sep=0.75pt]  [font=\LARGE,rotate=-0.71] [align=left] {$\displaystyle \ent{\X, \Xnew}$};
%		% Text Node
%		\draw (149.5,326.22) node [anchor=north west][inner sep=0.75pt]  [font=\LARGE,color={rgb, 255:red, 65; green, 117; blue, 5 }  ,opacity=1 ] [align=left] {$\displaystyle \ent{\Xnew}$};
%		
%	\end{tikzpicture}
%	}
%	\caption{Illustration of the augmented problem as an information diagram. The area of each circle represents the entropy value of a subset of variables. The mutual areas represent the MI values between these subsets. The diagram is constructed by taking into account that there isn't a mutual area between $\Xnot$ and both $\Xnew$, $\Z$ given $\Xinv$. The dark gray area is $\mi{\Xinv,\Xnew}{\Z}$, the light gray area is $\ent{\Xnew \mid \Xinv}$. Subtraction of the dark gray area by the light gray area yields the augmented MI. \GR{[change colors to match fig.1, increase text size, split into 2]}
%	}
%	\label{fig:augmented_info_diag}
%\end{figure}

% Information diagram
\begin{figure}
	\centering
	\begin{subfigure}[b]{0.49\textwidth}
		\centering
		\scalebox{0.22}{
			\includegraphics{info_diag_1}
		}
		\caption{}
		\label{fig:info_diag_1}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.49\textwidth}
		\centering
		\scalebox{0.22}{
			\includegraphics{info_diag_2}
		}
		\caption{}
		\label{fig:info_diag_2}
	\end{subfigure}
	\caption{Illustration of the augmented problem as an information diagram. The area of each circle represents the entropy value of a subset of variables. The mutual areas represent the MI values between these subsets. The key idea, obtained by Theorem~\ref{th:mi_aug_involved}, is that there is no mutual area between $\Xnot$ and both $\Xnew$, $\Z$ given $\Xinv$. The dark gray area in (a) is $\mi{\Xinv,\Xnew}{\Z}$, the light gray area in (b) is $\ent{\Xnew \mid \Xinv}$. Subtraction of the dark gray area by the light gray area yields the augmented MI. \vspace{-15pt}
	}
	\label{fig:augmented_info_diag}
\end{figure}




%% Information diagram
%\begin{figure}
%	\centering
%	\begin{subfigure}[b]{0.5\textwidth}
%			\scalebox{0.45}{
%			\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%				%uncomment if require: \path (0,461); %set diagram left start at 0, and has height of 461
%				
%				%Shape: Circle [id:dp7574015397150171] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.3 ] (335,326.74) .. controls (335,302.44) and (354.7,282.74) .. (379,282.74) .. controls (403.3,282.74) and (423,302.44) .. (423,326.74) .. controls (423,351.04) and (403.3,370.74) .. (379,370.74) .. controls (354.7,370.74) and (335,351.04) .. (335,326.74) -- cycle ;
%				%Shape: Circle [id:dp4888817328370705] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.3 ] (208,279.74) .. controls (208,255.44) and (227.7,235.74) .. (252,235.74) .. controls (276.3,235.74) and (296,255.44) .. (296,279.74) .. controls (296,304.04) and (276.3,323.74) .. (252,323.74) .. controls (227.7,323.74) and (208,304.04) .. (208,279.74) -- cycle ;
%				%Shape: Square [id:dp48085999986383743] 
%				\draw   (157,80) -- (513,80) -- (513,436) -- (157,436) -- cycle ;
%				%Shape: Circle [id:dp46404033827532687] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 84; blue, 255 }  ,fill opacity=1 ] (233.52,263.74) .. controls (233.52,260.57) and (236.09,258) .. (239.26,258) .. controls (242.43,258) and (245,260.57) .. (245,263.74) .. controls (245,266.91) and (242.43,269.48) .. (239.26,269.48) .. controls (236.09,269.48) and (233.52,266.91) .. (233.52,263.74) -- cycle ;
%				%Shape: Star [id:dp7527654107368411] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (329.94,238.99) -- (333.07,252.02) -- (346.36,250.98) -- (335,258) -- (340.09,270.39) -- (329.94,261.7) -- (319.79,270.39) -- (324.88,258) -- (313.52,250.98) -- (326.81,252.02) -- cycle ;
%				%Shape: Circle [id:dp9899652401244217] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ] (341.52,238.74) .. controls (341.52,235.57) and (344.09,233) .. (347.26,233) .. controls (350.43,233) and (353,235.57) .. (353,238.74) .. controls (353,241.91) and (350.43,244.48) .. (347.26,244.48) .. controls (344.09,244.48) and (341.52,241.91) .. (341.52,238.74) -- cycle ;
%				%Shape: Circle [id:dp28292812323162275] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ] (459.52,388.74) .. controls (459.52,385.57) and (462.09,383) .. (465.26,383) .. controls (468.43,383) and (471,385.57) .. (471,388.74) .. controls (471,391.91) and (468.43,394.48) .. (465.26,394.48) .. controls (462.09,394.48) and (459.52,391.91) .. (459.52,388.74) -- cycle ;
%				%Shape: Circle [id:dp14365046551032745] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ] (433.52,241.74) .. controls (433.52,238.57) and (436.09,236) .. (439.26,236) .. controls (442.43,236) and (445,238.57) .. (445,241.74) .. controls (445,244.91) and (442.43,247.48) .. (439.26,247.48) .. controls (436.09,247.48) and (433.52,244.91) .. (433.52,241.74) -- cycle ;
%				%Shape: Circle [id:dp39084257739298134] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ] (308.52,201.74) .. controls (308.52,198.57) and (311.09,196) .. (314.26,196) .. controls (317.43,196) and (320,198.57) .. (320,201.74) .. controls (320,204.91) and (317.43,207.48) .. (314.26,207.48) .. controls (311.09,207.48) and (308.52,204.91) .. (308.52,201.74) -- cycle ;
%				%Shape: Circle [id:dp7785143515038924] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ] (355.52,177.74) .. controls (355.52,174.57) and (358.09,172) .. (361.26,172) .. controls (364.43,172) and (367,174.57) .. (367,177.74) .. controls (367,180.91) and (364.43,183.48) .. (361.26,183.48) .. controls (358.09,183.48) and (355.52,180.91) .. (355.52,177.74) -- cycle ;
%				%Shape: Circle [id:dp060556128322981406] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ] (277.52,143.74) .. controls (277.52,140.57) and (280.09,138) .. (283.26,138) .. controls (286.43,138) and (289,140.57) .. (289,143.74) .. controls (289,146.91) and (286.43,149.48) .. (283.26,149.48) .. controls (280.09,149.48) and (277.52,146.91) .. (277.52,143.74) -- cycle ;
%				%Shape: Circle [id:dp7958598751803392] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ] (380.52,121.74) .. controls (380.52,118.57) and (383.09,116) .. (386.26,116) .. controls (389.43,116) and (392,118.57) .. (392,121.74) .. controls (392,124.91) and (389.43,127.48) .. (386.26,127.48) .. controls (383.09,127.48) and (380.52,124.91) .. (380.52,121.74) -- cycle ;
%				%Shape: Circle [id:dp716216946891977] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ] (435.52,149.74) .. controls (435.52,146.57) and (438.09,144) .. (441.26,144) .. controls (444.43,144) and (447,146.57) .. (447,149.74) .. controls (447,152.91) and (444.43,155.48) .. (441.26,155.48) .. controls (438.09,155.48) and (435.52,152.91) .. (435.52,149.74) -- cycle ;
%				%Shape: Circle [id:dp9575421361853615] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ] (199.52,375.74) .. controls (199.52,372.57) and (202.09,370) .. (205.26,370) .. controls (208.43,370) and (211,372.57) .. (211,375.74) .. controls (211,378.91) and (208.43,381.48) .. (205.26,381.48) .. controls (202.09,381.48) and (199.52,378.91) .. (199.52,375.74) -- cycle ;
%				%Shape: Circle [id:dp04976710197739176] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ] (187.52,177.74) .. controls (187.52,174.57) and (190.09,172) .. (193.26,172) .. controls (196.43,172) and (199,174.57) .. (199,177.74) .. controls (199,180.91) and (196.43,183.48) .. (193.26,183.48) .. controls (190.09,183.48) and (187.52,180.91) .. (187.52,177.74) -- cycle ;
%				%Shape: Circle [id:dp06365557602368432] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 84; blue, 255 }  ,fill opacity=1 ] (407.52,314.74) .. controls (407.52,311.57) and (410.09,309) .. (413.26,309) .. controls (416.43,309) and (419,311.57) .. (419,314.74) .. controls (419,317.91) and (416.43,320.48) .. (413.26,320.48) .. controls (410.09,320.48) and (407.52,317.91) .. (407.52,314.74) -- cycle ;
%				%Shape: Circle [id:dp7948587711253894] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ] (198.52,125.74) .. controls (198.52,122.57) and (201.09,120) .. (204.26,120) .. controls (207.43,120) and (210,122.57) .. (210,125.74) .. controls (210,128.91) and (207.43,131.48) .. (204.26,131.48) .. controls (201.09,131.48) and (198.52,128.91) .. (198.52,125.74) -- cycle ;
%				%Shape: Circle [id:dp24115767178738667] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ] (247.52,192.74) .. controls (247.52,189.57) and (250.09,187) .. (253.26,187) .. controls (256.43,187) and (259,189.57) .. (259,192.74) .. controls (259,195.91) and (256.43,198.48) .. (253.26,198.48) .. controls (250.09,198.48) and (247.52,195.91) .. (247.52,192.74) -- cycle ;
%				%Shape: Circle [id:dp9680869721747944] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ] (453.52,307.74) .. controls (453.52,304.57) and (456.09,302) .. (459.26,302) .. controls (462.43,302) and (465,304.57) .. (465,307.74) .. controls (465,310.91) and (462.43,313.48) .. (459.26,313.48) .. controls (456.09,313.48) and (453.52,310.91) .. (453.52,307.74) -- cycle ;
%				%Shape: Circle [id:dp29205024209928787] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ] (292.52,344.74) .. controls (292.52,341.57) and (295.09,339) .. (298.26,339) .. controls (301.43,339) and (304,341.57) .. (304,344.74) .. controls (304,347.91) and (301.43,350.48) .. (298.26,350.48) .. controls (295.09,350.48) and (292.52,347.91) .. (292.52,344.74) -- cycle ;
%				%Shape: Circle [id:dp8193782173800817] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 84; blue, 255 }  ,fill opacity=1 ] (343.52,347.74) .. controls (343.52,344.57) and (346.09,342) .. (349.26,342) .. controls (352.43,342) and (355,344.57) .. (355,347.74) .. controls (355,350.91) and (352.43,353.48) .. (349.26,353.48) .. controls (346.09,353.48) and (343.52,350.91) .. (343.52,347.74) -- cycle ;
%				%Shape: Circle [id:dp7929533609908146] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ] (252.52,391.74) .. controls (252.52,388.57) and (255.09,386) .. (258.26,386) .. controls (261.43,386) and (264,388.57) .. (264,391.74) .. controls (264,394.91) and (261.43,397.48) .. (258.26,397.48) .. controls (255.09,397.48) and (252.52,394.91) .. (252.52,391.74) -- cycle ;
%				%Shape: Circle [id:dp48685220843122945] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ] (420.52,188.74) .. controls (420.52,185.57) and (423.09,183) .. (426.26,183) .. controls (429.43,183) and (432,185.57) .. (432,188.74) .. controls (432,191.91) and (429.43,194.48) .. (426.26,194.48) .. controls (423.09,194.48) and (420.52,191.91) .. (420.52,188.74) -- cycle ;
%				%Shape: Circle [id:dp3878523346502083] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ] (377.52,410.74) .. controls (377.52,407.57) and (380.09,405) .. (383.26,405) .. controls (386.43,405) and (389,407.57) .. (389,410.74) .. controls (389,413.91) and (386.43,416.48) .. (383.26,416.48) .. controls (380.09,416.48) and (377.52,413.91) .. (377.52,410.74) -- cycle ;
%				%Shape: Circle [id:dp3504684817369763] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ] (489.52,110.74) .. controls (489.52,107.57) and (492.09,105) .. (495.26,105) .. controls (498.43,105) and (501,107.57) .. (501,110.74) .. controls (501,113.91) and (498.43,116.48) .. (495.26,116.48) .. controls (492.09,116.48) and (489.52,113.91) .. (489.52,110.74) -- cycle ;
%				%Shape: Circle [id:dp5052942263353948] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ] (238.52,93.74) .. controls (238.52,90.57) and (241.09,88) .. (244.26,88) .. controls (247.43,88) and (250,90.57) .. (250,93.74) .. controls (250,96.91) and (247.43,99.48) .. (244.26,99.48) .. controls (241.09,99.48) and (238.52,96.91) .. (238.52,93.74) -- cycle ;
%				%Shape: Circle [id:dp1760341954667266] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ] (307.52,413.74) .. controls (307.52,410.57) and (310.09,408) .. (313.26,408) .. controls (316.43,408) and (319,410.57) .. (319,413.74) .. controls (319,416.91) and (316.43,419.48) .. (313.26,419.48) .. controls (310.09,419.48) and (307.52,416.91) .. (307.52,413.74) -- cycle ;
%				%Shape: Circle [id:dp10277113938505567] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ] (338.52,105.74) .. controls (338.52,102.57) and (341.09,100) .. (344.26,100) .. controls (347.43,100) and (350,102.57) .. (350,105.74) .. controls (350,108.91) and (347.43,111.48) .. (344.26,111.48) .. controls (341.09,111.48) and (338.52,108.91) .. (338.52,105.74) -- cycle ;
%				%Shape: Circle [id:dp9541840415862923] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 84; blue, 255 }  ,fill opacity=1 ] (243.52,311.74) .. controls (243.52,308.57) and (246.09,306) .. (249.26,306) .. controls (252.43,306) and (255,308.57) .. (255,311.74) .. controls (255,314.91) and (252.43,317.48) .. (249.26,317.48) .. controls (246.09,317.48) and (243.52,314.91) .. (243.52,311.74) -- cycle ;
%				%Shape: Circle [id:dp5290688918826407] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 84; blue, 255 }  ,fill opacity=1 ] (368.52,296.74) .. controls (368.52,293.57) and (371.09,291) .. (374.26,291) .. controls (377.43,291) and (380,293.57) .. (380,296.74) .. controls (380,299.91) and (377.43,302.48) .. (374.26,302.48) .. controls (371.09,302.48) and (368.52,299.91) .. (368.52,296.74) -- cycle ;
%				%Shape: Circle [id:dp22386464873735523] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ] (169.52,336.74) .. controls (169.52,333.57) and (172.09,331) .. (175.26,331) .. controls (178.43,331) and (181,333.57) .. (181,336.74) .. controls (181,339.91) and (178.43,342.48) .. (175.26,342.48) .. controls (172.09,342.48) and (169.52,339.91) .. (169.52,336.74) -- cycle ;
%				%Shape: Circle [id:dp9861807702148508] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ] (157.52,245.74) .. controls (157.52,242.57) and (160.09,240) .. (163.26,240) .. controls (166.43,240) and (169,242.57) .. (169,245.74) .. controls (169,248.91) and (166.43,251.48) .. (163.26,251.48) .. controls (160.09,251.48) and (157.52,248.91) .. (157.52,245.74) -- cycle ;
%				%Shape: Circle [id:dp3306501854859958] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.5 ] (490.52,208.74) .. controls (490.52,205.57) and (493.09,203) .. (496.26,203) .. controls (499.43,203) and (502,205.57) .. (502,208.74) .. controls (502,211.91) and (499.43,214.48) .. (496.26,214.48) .. controls (493.09,214.48) and (490.52,211.91) .. (490.52,208.74) -- cycle ;
%				%Shape: Star [id:dp7613680136704071] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (379,317.03) -- (380.75,324.32) -- (388.19,323.74) -- (381.83,327.67) -- (384.68,334.6) -- (379,329.74) -- (373.32,334.6) -- (376.17,327.67) -- (369.81,323.74) -- (377.25,324.32) -- cycle ;
%				%Shape: Star [id:dp39726979379106164] 
%				\draw  [draw opacity=0][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (252,270.03) -- (253.75,277.32) -- (261.19,276.74) -- (254.83,280.67) -- (257.68,287.6) -- (252,282.74) -- (246.32,287.6) -- (249.17,280.67) -- (242.81,276.74) -- (250.25,277.32) -- cycle ;
%				%Curve Lines [id:da44135563986835824] 
%				\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (252,279.74) .. controls (293,289.48) and (302,286.48) .. (329.94,256.35) ;
%				%Curve Lines [id:da7544037942905801] 
%				\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (329.94,256.35) .. controls (378,280.48) and (349,311.48) .. (379,326.74) ;
%				
%		\end{tikzpicture}}
%	\end{subfigure}
%	\begin{subfigure}[b]{0.45\textwidth}
%		\centering
%			\scalebox{0.45}{
%			\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%				%uncomment if require: \path (0,441); %set diagram left start at 0, and has height of 441
%				
%				%Curve Lines [id:da4033650573064922] 
%				\draw [draw opacity=0][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.75] [line join = round][line cap = round]   (165.5,189.8) .. controls (165.5,183.8) and (170.62,183.12) .. (173.5,178.8) .. controls (175.01,176.54) and (174.83,173.46) .. (175.5,170.8) .. controls (176.2,167.99) and (183.3,162.47) .. (185.5,158.8) .. controls (192.5,150.8) and (197.5,147.8) .. (206.5,141.8) .. controls (211.5,137.8) and (223.4,132.98) .. (230.5,131.8) .. controls (239.5,126.8) and (247.15,128.67) .. (256.5,126.8) .. controls (266.92,124.72) and (284.5,127.8) .. (296.5,129.8) .. controls (298.26,130.68) and (285.99,133.68) .. (285.5,133.8) .. controls (282.28,134.61) and (278.83,136.93) .. (274.5,137.8) .. controls (265.5,143.8) and (256.28,154.02) .. (251.5,158.8) .. controls (248.48,161.82) and (243.87,163.25) .. (241.5,166.8) .. controls (240.1,168.9) and (240.79,173.51) .. (238.5,175.8) .. controls (231.12,183.18) and (225.8,204.07) .. (224.5,215.8) .. controls (223.33,226.37) and (223.5,237.8) .. (223.5,249.8) .. controls (223,251.53) and (218.13,245.9) .. (217.5,245.8) .. controls (209.8,244.52) and (205.71,239.06) .. (198.5,236.66) .. controls (192.5,229.8) and (191.52,227.82) .. (186.5,222.8) .. controls (178.18,214.48) and (173.85,209.85) .. (169.5,196.8) .. controls (168.22,192.95) and (164.5,192.46) .. (164.5,186.8) ;
%				%Curve Lines [id:da9329263652587878] 
%				\draw [draw opacity=0][pattern=_h3dylt67w,pattern size=6pt,pattern thickness=1.5pt,pattern radius=0pt, pattern color={rgb, 255:red, 0; green, 0; blue, 0}][line width=0.75] [line join = round][line cap = round]   (165.5,189.8) .. controls (165.5,183.8) and (170.62,183.12) .. (173.5,178.8) .. controls (175.01,176.54) and (174.83,173.46) .. (175.5,170.8) .. controls (176.2,167.99) and (183.3,162.47) .. (185.5,158.8) .. controls (192.5,150.8) and (197.5,147.8) .. (206.5,141.8) .. controls (211.5,137.8) and (223.4,132.98) .. (230.5,131.8) .. controls (239.5,126.8) and (247.15,128.67) .. (256.5,126.8) .. controls (266.92,124.72) and (284.5,127.8) .. (296.5,129.8) .. controls (298.26,130.68) and (285.99,133.68) .. (285.5,133.8) .. controls (282.28,134.61) and (278.83,136.93) .. (274.5,137.8) .. controls (265.5,143.8) and (256.28,154.02) .. (251.5,158.8) .. controls (248.48,161.82) and (243.87,163.25) .. (241.5,166.8) .. controls (240.1,168.9) and (240.79,173.51) .. (238.5,175.8) .. controls (231.12,183.18) and (225.8,204.07) .. (224.5,215.8) .. controls (223.33,226.37) and (223.5,237.8) .. (223.5,249.8) .. controls (223,251.53) and (218.13,245.9) .. (217.5,245.8) .. controls (209.8,244.52) and (205.71,239.06) .. (198.5,236.66) .. controls (192.5,229.8) and (191.52,227.82) .. (186.5,222.8) .. controls (178.18,214.48) and (173.85,209.85) .. (169.5,196.8) .. controls (168.22,192.95) and (164.5,192.46) .. (164.5,186.8) ;
%				%Curve Lines [id:da4421168531852726] 
%				\draw [draw opacity=0][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ][line width=0.75] [line join = round][line cap = round]   (166.5,193.66) .. controls (166.83,196.66) and (166.85,199.71) .. (167.5,202.66) .. controls (167.78,203.91) and (172.66,206.82) .. (174.5,208.66) .. controls (182.11,216.27) and (189.77,227.93) .. (198.5,236.66) .. controls (201.25,239.4) and (208.99,239.15) .. (211.5,241.66) .. controls (213.1,243.26) and (216.76,246.92) .. (218.5,248.66) .. controls (219.81,249.96) and (226.3,251.66) .. (226.5,252.66) .. controls (227.16,255.94) and (224.3,259.53) .. (225.5,262.66) .. controls (228.67,270.89) and (229.7,267.92) .. (233.7,275.92) .. controls (236.41,278.63) and (240.7,286.92) .. (237.5,281.66) .. controls (238.52,285.74) and (243.65,289.81) .. (246.5,292.66) .. controls (247.92,294.08) and (242.9,291.18) .. (250.7,296.92) .. controls (253.9,302.18) and (253.13,300.92) .. (254.5,303.66) .. controls (256.61,307.87) and (263.33,314.57) .. (269.5,317.66) .. controls (271.68,318.75) and (276.43,321.52) .. (277.5,321.66) .. controls (280.17,321.99) and (283.6,320.76) .. (285.5,322.66) .. controls (286.33,323.48) and (292.54,324.6) .. (291.5,324.66) .. controls (276.98,325.51) and (277.67,326.04) .. (265.79,327.12) .. controls (261.36,327.53) and (256.16,329.82) .. (251.5,328.66) .. controls (250.78,328.48) and (251.22,326.84) .. (250.5,326.66) .. controls (244.63,325.19) and (236,325.39) .. (230.5,324.66) .. controls (228.4,324.38) and (225.75,320.59) .. (222.5,319.66) .. controls (219.47,318.79) and (216.34,319.79) .. (213.5,318.66) .. controls (202.64,314.31) and (192.39,303.54) .. (183.5,294.66) .. controls (179.27,290.43) and (176,288.55) .. (173.79,284.12) .. controls (175.07,282.59) and (169.96,274.03) .. (168.5,269.66) .. controls (168.05,268.31) and (165.84,268.03) .. (165.5,266.66) .. controls (163.69,259.43) and (164.06,254.46) .. (162.5,246.66) .. controls (161.82,243.25) and (158.71,241.56) .. (158.5,238.66) .. controls (157.86,229.74) and (160.82,218.76) .. (161.5,212.66) .. controls (162.14,206.93) and (161.5,201.65) .. (163.5,197.66) .. controls (163.97,196.71) and (164.5,193.6) .. (164.5,194.66) .. controls (164.5,195.4) and (164.75,196.66) .. (165.5,196.66) ;
%				%Curve Lines [id:da2780428942483901] 
%				\draw [draw opacity=0][fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ][line width=0.75] [line join = round][line cap = round]   (294.1,129.34) .. controls (312.34,123.26) and (330.69,124.24) .. (347.1,128.34) .. controls (352.21,129.62) and (356.9,129.29) .. (361.1,130.34) .. controls (361.82,130.52) and (363.05,130.59) .. (363.1,131.34) .. controls (363.46,136.41) and (362.53,152.79) .. (362.1,158.34) .. controls (361.59,164.99) and (361.45,171.67) .. (361.1,178.34) .. controls (360.86,182.85) and (354.23,187.83) .. (353.1,192.34) .. controls (350.52,202.65) and (341.1,214.34) .. (334.1,225.34) .. controls (326.67,229.05) and (319.98,240.12) .. (311.1,242.34) .. controls (307.41,243.26) and (299.1,249.34) .. (295.1,248.34) .. controls (291.28,250.25) and (283.93,252.42) .. (280.1,254.34) .. controls (268.84,259.97) and (247.45,253.71) .. (235.1,252.34) .. controls (234.15,252.23) and (229.29,248.7) .. (227.1,248.34) .. controls (226.16,248.18) and (221.58,251.23) .. (221.1,248.34) .. controls (221.1,233.34) and (219.81,241.06) .. (220.1,237.34) .. controls (221.05,225.01) and (222.76,214.04) .. (225.1,202.34) .. controls (226.4,195.83) and (229.71,191.12) .. (233.1,184.34) .. controls (234.39,181.75) and (234.1,177.93) .. (235.1,175.34) .. controls (238.46,166.61) and (244.19,161.28) .. (250.1,157.34) .. controls (256.1,153.34) and (265.94,145.5) .. (270.1,141.34) .. controls (274.11,137.33) and (292.99,128.34) .. (299.1,128.34) ;
%				%Shape: Ellipse [id:dp604915699384222] 
%				\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=4.5]  (310.9,292.95) .. controls (276.21,249.36) and (284.05,185.4) .. (328.42,150.1) .. controls (372.79,114.79) and (436.87,121.51) .. (471.56,165.11) .. controls (506.25,208.7) and (498.41,272.66) .. (454.04,307.97) .. controls (409.67,343.27) and (345.59,336.55) .. (310.9,292.95) -- cycle ;
%				%Shape: Ellipse [id:dp14907252596438347] 
%				\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=4.5]  (243.44,291.46) .. controls (208.75,247.87) and (216.59,183.91) .. (260.96,148.6) .. controls (305.33,113.3) and (369.41,120.02) .. (404.1,163.62) .. controls (438.79,207.21) and (430.95,271.17) .. (386.58,306.47) .. controls (342.21,341.78) and (278.13,335.06) .. (243.44,291.46) -- cycle ;
%				%Shape: Brace [id:dp22614282606535463] 
%				\draw   (171.24,380.67) .. controls (171.24,385.34) and (173.57,387.67) .. (178.24,387.67) -- (320.61,387.67) .. controls (327.28,387.67) and (330.61,390) .. (330.61,394.67) .. controls (330.61,390) and (333.94,387.67) .. (340.61,387.67)(337.61,387.67) -- (482.97,387.67) .. controls (487.64,387.67) and (489.97,385.34) .. (489.97,380.67) ;
%				%Shape: Ellipse [id:dp8015781431346674] 
%				\draw  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=4.5]  (180.44,291.46) .. controls (145.75,247.87) and (153.59,183.91) .. (197.96,148.6) .. controls (242.33,113.3) and (306.41,120.02) .. (341.1,163.62) .. controls (375.79,207.21) and (367.95,271.17) .. (323.58,306.47) .. controls (279.21,341.78) and (215.13,335.06) .. (180.44,291.46) -- cycle ;
%				%Shape: Ellipse [id:dp2165364938533929] 
%				\draw  [color={rgb, 255:red, 248; green, 231; blue, 28 }  ,draw opacity=1 ][line width=4.5]  (180.63,218.53) .. controls (145.94,174.93) and (153.78,110.97) .. (198.15,75.67) .. controls (242.52,40.36) and (306.6,47.09) .. (341.29,90.68) .. controls (375.98,134.27) and (368.14,198.23) .. (323.77,233.54) .. controls (279.4,268.84) and (215.32,262.12) .. (180.63,218.53) -- cycle ;
%				%Curve Lines [id:da8868483261943054] 
%				\draw [line width=2.25]    (278.79,197.27) .. controls (272.1,174.6) and (222.1,142.6) .. (193.1,176.6) .. controls (164.97,209.58) and (133.08,198.34) .. (109.28,154.74) ;
%				\draw [shift={(107.1,150.6)}, rotate = 422.95] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%				%Curve Lines [id:da8485677356785608] 
%				\draw [line width=2.25]    (212.79,287.12) .. controls (201.79,255.12) and (170.1,248.6) .. (141.1,282.6) .. controls (112.68,315.92) and (82.04,249.86) .. (51.65,306.5) ;
%				\draw [shift={(49.79,310.12)}, rotate = 296.2] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%				%Curve Lines [id:da23185241288128777] 
%				\draw [line width=2.25]    (210.1,212.45) .. controls (171.1,227.45) and (170.1,248.6) .. (141.1,282.6) ;
%				%Curve Lines [id:da058373919020516585] 
%				\draw [line width=2.25]    (219.1,197.65) .. controls (201.1,181.65) and (196.1,189.65) .. (164.5,194.66) ;
%				
%				% Text Node
%				\draw (169.5,39.99) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 248; green, 231; blue, 28 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{28.95pt}\setlength\topsep{0pt}
%						\begin{center}
%							$\displaystyle \ent{\Z}$
%						\end{center}
%						
%				\end{minipage}};
%				%% Text Node
%				\draw (32,125.2) node [anchor=north west][inner sep=0.75pt]   [align=left] {
%					\textcolor[rgb]{0.29,0.29,0.29}{
%						$\begin{aligned}
%							\mi{\Xinv, \Xnew}{Z}
%						\end{aligned}$}};
%				%% Text Node
%				\draw (3,314.2) node [anchor=north west][inner sep=0.75pt]   [align=left] {
%					\textcolor[rgb]{0.61,0.61,0.61}{
%						$\begin{aligned}
%							\ent{\Xnew \mid \X} = \\ 
%							\ent{\Xnew \mid \Xinv}
%						\end{aligned}$}};
%				% Text Node
%				\draw (384.5,344.22) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ] [align=left] {$\displaystyle \ent{\Xnot}$};
%				% Text Node
%				\draw (293.5,345.22) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ] [align=left] {$\displaystyle \ent{\Xinv}$};
%				% Text Node
%				\draw (307.23,404.23) node [anchor=north west][inner sep=0.75pt]  [rotate=-0.71] [align=left] {$\displaystyle \ent{\X, \Xnew}$};
%				% Text Node
%				\draw (209.5,346.22) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,opacity=1 ] [align=left] {$\displaystyle \ent{\Xnew}$};
%		\end{tikzpicture}}
%		%		\caption{Standard deviation of MI with increasing state dimensionality}
%		\caption{}
%		\label{fig:std_with_dimension}
%	\end{subfigure}
%
%	\caption{\VI{[try]}}
%	\label{fig:augmented_info_diag}
%\end{figure}


%The involved variables depend on the specific action and its observations. Reasoning about the exact involved variables of each action and marginalizing out the uninvolved variables for each action might be costly operations which will eventually make this whole approach worthless. It is easy to show that
%% TODO: \GR{[how?]}
%if we choose a subset $\Xinvp$ which contains the involved variables but might also contain some other uninvolved variables, so that $\Xinv \subseteq \Xinvp \subseteq \X$, then Theorem~\ref{th:mi_aug_involved} can be written more generally as
%%
%\begin{equation}
%\miaug{\X}{\Xnew}{\Z} = \miaug{\Xinvp}{\Xnew}{\Z},
%\end{equation}
%%
%meaning that it is sufficient to choose a subset \emph{containing} the involved rather than \emph{only} the involved. This subset has larger dimensions, yet it might still be much smaller in dimensions compared to the whole state. This result will be helpful in case we have an easy way to calculate marginalized beliefs of subsets which are not exactly the involved but contain them. Also, if we have $n$ candidate actions, denoting the involved subset for the $j$-th action as $\Xinvi{j}$ and choosing $\Xinvp = \Xinvi{1} \cup \Xinvi{2} \cup \dots \cup \Xinvi{n}$, will result in a one-time marginalization rather then marginalizing for each action separately. This concept is similar to the one suggested in \cite{Kopitkov17ijrr}. We will continue to refer to $\Xinv$ rather than $\Xinvp$ for readability reasons, yet we emphasize that the following is true for $\Xinvp$ as well.


\begin{wrapfigure}{r}{7.5cm}
	\vspace{-20pt}
	\begin{minipage}{\textwidth}
		\begin{algorithm}[H]
			\caption{\invmi{}}
			\label{alg:invmi}
			\scriptsize
			\begin{algorithmic}[1]
				\Require $\bel{\X}$, $\FT$, $\FZ$, $a$
				\Ensure $\miaug{\X}{\Xnew}{\Z}$
				\State $\Xinv \gets$ \Call{DetermineInvolved}{$\bel{\X}, \FT, \FZ, a$}
				\State $\bel{\Xinv} \gets$ \Call{Marginalize}{$\bel{\X}, \Xinv$}
				\State $\miaug{\Xinv}{\Xnew}{\Z} \gets$ \Call{CalcMI}{$\bel{\Xinv}, \FT, \FZ, a$} 
				%				\Comment{any calculation scheme}
				\State $\miaug{\X}{\Xnew}{\Z} \gets \miaug{\Xinv}{\Xnew}{\Z}$
			\end{algorithmic}
		\end{algorithm}
	\end{minipage}
	\vspace{-20pt}
\end{wrapfigure}

Using the result of Theorem \ref{th:mi_aug_involved}, we propose an approach which we will refer to as \invmi{}, and is summarized in Algorithm~\ref{alg:invmi}. Given the prior belief, the probabilistic models and an action sequence, this algorithm first determines the involved variables using some heuristic. Then, it calculates the marginalized prior belief over the involved variables. And, finally, it calculates the (augmented) MI value using the marginalized prior belief (while propagating future beliefs), using any calculation scheme. This is instead of naively using the entire prior belief.
We remind that either or both the complexity and the accuracy of any calculation scheme of the MI depend on the dimension of the entire state, $D$. The \emph{main contribution} of our approach is that it cancels this dependence. Instead, the dependence is over the dimension of a smaller subset of the state, $d$, which improves either or both the complexity and the accuracy.
In order to make the overall marginalization process more efficient, we can instead work with $\Xinvp$, and the algorithm is then slightly changed depending on how it is defined, yet the key idea remains the same.

%\add{
%The approach presented, which we will refer to as \invmi{}, is concluded in Algorithm~\ref{alg:invmi}. Given the prior belief, the probabilistic models and an action sequence, this algorithm first determines the involved variables using some heuristic. Then, it calculates the marginalized prior belief over the involved. And, finally, it calculates the (augmented) MI value using the marginalized prior belief, \GR{while propagating the beliefs. This is} instead of naively using the entire prior belief.
%We remind that either or both the complexity and the accuracy of any calculation scheme of the MI depend on the dimension of the state, $D$. The main contribution of our approach is that it cancels this dependence and switches it to dependence over the dimension of a smaller subset of the state, $d$, thus improving either or both the complexity and the accuracy.
%We emphasize again that $\Xinvp$ might be used instead of $\Xinv$, a case for which the algorithm slightly changes depending on how it is defined, but the key idea remains the same.
%}
% TODO: look at the paper vadim sent me regarding the determination of involved

%\begin{algorithm}
%	\caption{\invmi{}}
%	\label{alg:invmi}
%	\scriptsize
%	\begin{algorithmic}[1]
%		\Require $\bel{\X}$, $\FT$, $\FZ$, $a$
%		\Ensure $\miaug{\X}{\Xnew}{\Z}$
%		\State $\Xinv \gets$ \Call{DetermineInvolved}{$\bel{\X}, \FT, \FZ, a$}
%		\State $\bel{\Xinv} \gets$ \Call{Marginalize}{$\bel{\X}, \Xinv$}
%		\State $\miaug{\Xinv}{\Xnew}{\Z} \gets$ \Call{CalcMI}{$\bel{\Xinv}, \FT, \FZ, a$} // any calculation scheme
%		\State $\miaug{\X}{\Xnew}{\Z} \gets \miaug{\Xinv}{\Xnew}{\Z}$
%	\end{algorithmic}
%\end{algorithm}



Note also this approach is not limited to any specific calculation scheme of the MI. The calculation, for example, might go through its relation to entropy, by calculating the entropy terms or estimating them using entropy estimators, such as the common re-substitution estimator with KDE we have briefly introduced in Section \ref{sec:problem-formulation}.
We shall use it now to demonstrate the complexity reduction we get from using our approach. It is easy to first see that for the same number of samples, our approach reduces the complexity of estimating the entropy terms from $O \left( N^2 D \right)$ to $O \left( N^2 d \right)$. However, as we have already mentioned, the Curse of Dimensionality suggests that the number of samples required to get the same accuracy is exponential in the dimension. Thus, if we wish to preserve the accuracy, using our approach, only $n \propto \alpha^d$ samples are required, compared to $N \propto \alpha^D$ samples which were required without our approach. Since $d \ll D$, it means that $n \ll N$. This reduces the complexity even further to $O \left( n^2 d \right)$. To generalize and simplify our conclusion, we consider the complexity of any estimator is at least linear in the number of samples, thus the complexity is reduced, at least, from $O \left( \alpha^{D} \right)$ to $O \left( \alpha^{d} \right)$, where we remind that $d \ll D$ and $\alpha \geq 1$.
%\add{
%Given the \GR{(unified)} marginalized prior belief $\bel{\Xinv}$ and the problem's models, we can then, as commonly done, construct a belief tree, by using any arbitrary inference engine to infer future posterior beliefs (the nodes of the tree). 
%%use any arbitrary inference engine to infer $m$ future observations instances $\{ \z{i} \}_{i=1}^m$ and a posterior future belief $\bel{\Xinv, \Xnew \mid \z{i}}$ for each such observation instance.
%The entropy terms in eq.~(\ref{eq:mi_aug_inv_def}) can then be estimated with any estimator, such as the KDE re-substitution estimator we have introduced in section \ref{subsec:nonpara_ent_est}. The main idea, which is also the main contribution of our approach, is that no matter the inference engine nor entropy estimator, these entropy terms are estimated over a much lower-dimensional subset of the state rather than its entirety.
%}
%% TODO: add another equation which shows this estimation, by averaging over future observations
%% TODO: talk about the possibility to marginalize for any action or marginalize once for all actions

%\add{
%\GR{[rephrase and think where to put. Also state that it is for a re-substitution estimator]} Given that the number of samples is the same, we will get a better accuracy \GR{[Can be shown mathematically?]}. of calculating each entropy value (for each observation value), our approach is also better, $O \left( N^2 d \right)$ compared to $O \left( N^2 D \right)$ for the naive approach, where we remind that usually $d \ll D$. Given that we only wish to preserve the accuracy, less samples would be required ($n < N$) \GR{[Can this be shown mathematically?]}, reducing the complexity even further to $O \left( n^2 d \right)$. Considering a total number of $m$ observations instances, the complexity of estimating the MI eventually becomes $O \left( m n^2 d \right)$.
%}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Avoiding the reconstruction of future beliefs' surfaces} \label{subsec:no_kde}

The estimation scheme of the involved MI might require reconstructing the surfaces of future beliefs, which adds to the estimation error or perhaps entails another level of complexity in the form of new hyperparameters.
In this section, we present a theoretical derivation that allows to avoid this reconstruction step for the augmented MI calculation. We then use this derivation to construct an estimator.
This estimator, however, as will shortly be explained, can only be used in cases in which the probabilistic models are explicitly given. 
%
\begin{theorem}
	\label{th:mi_augmented_superposition}
	Let \(\X\) be some prior state, and \(\X' = \left\{ \X, \Xnew \right\}\) be a successor state, where \(\Xnew\) is the augmented subset of the successor state. Let \(\Z\) be an observation sequence over a subset of the successor state, \( \left\{\Xinv, \Xnew \right\} \subseteq \X'\), such that \( \prob{\Z \mid \X, \Xnew} \equiv \prob{\Z \mid \Xinv, \Xnew} \). Then, the augmented MI can be factorized as
	\begin{equation}
		\label{equ:mi_augmented_superposition}
		\miaug{\X}{\Xnew}{\Z} = -\ent{\Xnew \mid \Xinv} - \ent{\Z \mid \Xinv, \Xnew} + \ent{\Z}.
	\end{equation}
\end{theorem}
%
This result suggests that the augmented MI can be expressed as a superposition of the expected entropies of the sequential transition model, observation model and normalizer. More explicitly, the augmented MI can be written as
\begin{equation}
	\label{eq:mi_augmented_integrals}
	\begin{aligned}
		\miaug{\X}{\Xnew}{\Z} &=
		\int_{\XinvSp} \bel{\Xinv} \left[ \int_{\XnewSp} \FT  \log \FT d\Xnew \right] d\Xinv \\
		&+ \int_{\XinvSp} \bel{\Xinv} \Bigg[ \int_{\XnewSp} \FT 
		\left[ \int_{\ZSp} \FZ \log \FZ d\Z \right] d\Xnew \Bigg] d\Xinv \\
		&- \int_{\XinvSp} \bel{\Xinv} \bigg[ \int_{\XnewSp} \FT 
		\left[ \int_{\ZSp} \FZ \log \eta^{-1} d\Z \right] d\Xnew \bigg] d\Xinv,
	\end{aligned}
\end{equation}
where the normalizer can be calculated with
\begin{equation}
	\label{eq:normalizer}
	\eta^{-1} =
	\int_{\XinvSp} \bel{\Xinv} \left[ \int_{\XnewSp} \FT \FZ d\Xnew \right] d\Xinv.
\end{equation}
Eqs.~\eqref{eq:mi_augmented_integrals} and \eqref{eq:normalizer} suggest that the objective function can be calculated without the need to reconstruct future beliefs' surfaces, which is a \emph{key result}. Also, the integration is over the involved and new variables, already exploiting the dimensionality reduction.

%\VI{
%Using the definition of entropy and the notations of the sequential models from (\ref{eq:sequential_models}), the first term on the right hand side of eq.~(\ref{equ:mi_augmented_superposition}) becomes
%%
%\begin{equation}
%\begin{gathered}
%	\ent{\Xnew \mid \Xinv} =
%	- \int_{\XinvSp} \bel{\Xinv} \left[ \int_{\XnewSp} \FT  \log \FT d\Xnew \right] d\Xinv.
%\end{gathered}
%\end{equation}
%%
%Doing the same for the second term of eq.~(\ref{equ:mi_augmented_superposition}) yields
%%
%\begin{equation}
%\begin{gathered}
%	\ent{\Z \mid \Xinv, \Xnew} =
%	- \int_{\XinvSp} \bel{\Xinv} \Bigg[ \int_{\XnewSp} \FT 
%	\left[ \int_{\ZSp} \FZ \log \FZ d\Z \right] d\Xnew \Bigg] d\Xinv.
%\end{gathered}
%\end{equation}
%%
%And, lastly, the third term in eq.~(\ref{equ:mi_augmented_superposition}) is defined by
%%
%\begin{equation}
%\label{eq:z_entropy}
%\ent{\Z} =
%- \int_{\ZSp} \eta^{-1} \log \eta^{-1} d\Z,
%\end{equation}
%%
%where we can use the law of total probability to get
%%
%\begin{equation}
%\eta^{-1} =
%\int_{\XinvSp} \bel{\Xinv} \left[ \int_{\XnewSp} \FT \FZ d\Xnew \right] d\Xinv.
%\end{equation}
%%
%Plugging this back into eq.~(\ref{eq:z_entropy}) and changing integration order yields
%%
%\begin{equation}
%\begin{aligned}
%	\ent{\Z} = 
%	- \int_{\XinvSp} \bel{\Xinv} \bigg[ \int_{\XnewSp} \FT 
%	\left[ \int_{\ZSp} \FZ \log \eta^{-1} d\Z \right] d\Xnew \bigg] d\Xinv.
%\end{aligned}
%\end{equation}
%%
%The above analysis provides an exact formulation for the calculation of the augmented MI over a high-dimensional state that only involves integration over the involved variables, for any of the terms, including $\eta^{-1}$.
%Also, any of these terms can be expressed by only using the prior belief and the probabilistic models, assuming these are explicitly given. Thus, without explicitly requiring the posterior belief, the reconstruction step can be avoided.
%Plugging these terms back into eq.~(\ref{equ:mi_augmented_superposition}) and using sampling, i.e.
%%
%\begin{equation}
%\begin{gathered}
%	\xinv{i} \sim \bel{\Xinv} \\
%	\xnew{i,j} \sim \FT \left( \Xnew \mid \xinv{i} \right) \\
%	\zz{i,j,k} \sim \FZ \left( \Z \mid \xinv{i}, \xnew{i,j} \right),
%\end{gathered}
%\end{equation}
%%
%the augmented MI is approximated as
%%
%\begin{equation}
%\begin{gathered}
%	\miaug{\X}{\Xnew}{\Z} \approx
%	\sum_{i=1}^{n_1} w^{(i)} \left[ \frac{1}{n_2} \sum_{j=1}^{n_2} \log \FT^{(i,j)} \right] \\
%	+ \sum_{i=1}^{n_1} w^{(i)} \left[ \frac{1}{n_2} \sum_{j=1}^{n_2} \left[ \frac{1}{n_3} \sum_{k=1}^{n_3} \log \FZ^{(i,j,k)} \right] \right] \\
%	- \sum_{i=1}^{n_1} w^{(i)} \left[  \frac{1}{n_2} \sum_{j=1}^{n_2} \left[ \frac{1}{n_3} \sum_{k=1}^{n_3} \log {\eta^{-1}}^{(i,j,k)} \right] \right],
%\end{gathered}
%\end{equation}
%%
%where
%%
%\begin{equation}
%\begin{gathered}
%	\FT^{(i,j)} = \FT \left( \xinv{i}, \xnew{i,j} \right) \\
%	\FZ^{(i,j,k)} = \FZ \left( \xinv{i}, \xnew{i,j}, \zz{i,j,k} \right) \\
%	{\eta^{-1}}^{(i,j,k)} = \eta^{-1} \left( \xinv{i}, \xnew{i,j}, \zz{i,j,k} \right),
%\end{gathered}
%\end{equation}
%%
%and the normalizer, for each sampled instance, is then also approximated as
%%
%\begin{equation}
%{\eta^{-1}}^{(i,j,k)} \approx
%\sum_{l=1}^{n_4} w^{(l)} \left[ \frac{1}{n_5} \sum_{m=1}^{n_5} \FZ^{(l,m,k)} \right].
%\end{equation}
%%
%[Reduce drastically]}

%As in a particle filter, $\FZ^{(l,m,k)}$ can be considered an update for the particle's weight. Thus, the approximation of ${\eta^{-1}}^{(i,j,k)}$ can be viewed as an average of the updated weights.

We then use sampling to estimate eqs.~\eqref{eq:mi_augmented_integrals} and \eqref{eq:normalizer}, as summarized  in Algorithm~\ref{alg:invmi-smc}. The full details can be found in Appendix \ref{sec:Developing-estimator}. % Section 3.2 in the supplementary material.
%This estimation scheme is concluded in Algorithm~\ref{alg:invmi-smc}.
Since it uses particles from the prior and propagates them as in Sequential Monte Carlo (SMC) methods, we will refer to it as \mismc{}.
Note that this algorithm can be an \emph{anytime} algorithm, since the calculation can be updated incrementally when adding more particles.
% Note that this formulation allows the algorithm to be an \emph{anytime} algorithm. \GR{Given that we have a limited time for each planning step, we can start with a small set of particles and incrementally refine the calculation by increasing the number of particles until the time is up, without the need to calculate from scratch whenever more samples are added. [remove maybe? it is the meaning of anytime, which should be clear...]}
%This might not always be possible using other estimation schemes.

%\VI{
%The presented estimator might seem at a first glance very similar to the estimator in \cite{Boers10fusion}, although \mismc{} calculates MI and \cite{Boers10fusion} calculates entropy. Both use samples from the prior belief, propagates them and calculate entropy/MI without the reconstruction of future belief's surfaces. However, the key difference is the problem formulation these two address. Whereas in our work we treat a smoothing formulation, \cite{Boers10fusion} treats a filtering formulation. A filtering formulation means marginalizing out past states, which eventually makes the entire state involved, thus \cite{Boers10fusion} cannot be scaled to high-dimensional problems compared to our approach.
%[can be reduced/omitted if needed]}
% TODO: not sure this explanation holds

Also note that although this estimator is formulated by already exploiting the dimensionality reduction, it is not vital. The estimator can get as an input the full prior belief $\bel{\X}$ instead of the involved prior belief $\bel{\Xinv}$. The particles would then be high-dimensional, yet since these are used only for the evaluation of the probabilistic models, marginalization would automatically be done in the context of these particles. This attribute makes this estimator closely related to the \invmi{} approach, without explicitly using it beforehand. However, to avoid the Curse of Dimensionality, it is preferred to maintain and sample from a lower-dimensional belief to begin with, which is exactly the result of using \invmi{}.
% \VI{[clarify this is what we get with involve-MI]}.

	
%\begin{algorithm}[h]
%	\caption{\mismc}
%	\label{alg:invmi-smc}
%	\scriptsize
%	\begin{algorithmic}[1]
%		\Require $\bel{\Xinv}$, $\FT$, $\FZ$, $a$
%		\Ensure $\miaug{\Xinv}{\Xnew}{\Z}$
%		\State $sum_1 \gets 0$
%		\State $sum_2 \gets 0$
%		\State $sum_3 \gets 0$
%		\For{$i=1$ \textbf{to} $n_1$}
%		\State $\left(\xinv{i},w^{(i)} \right) \sim \bel{\Xinv}$
%		\For{$j=1$ \textbf{to} $n_2$}
%		\State $\xnew{i,j} \sim \FT(\Xnew \mid \xinv{i}, a)$
%		\State $value_1 \gets w^{(i)} \frac{1}{n_2} \log \FT^{(i,j)}$
%		\State $sum_1 \gets sum_1 + value_1$
%		\For{$k=1$ \textbf{to} $n_3$}
%		\State $\zz{i,j,k} \sim \FZ(\Z \mid \xinv{i}, \xnew{i,j})$
%		\State $value_2 \gets w^{(i)} \frac{1}{n_2} \frac{1}{n_3} \log \FZ^{(i,j,k)}$
%		\State $sum_2 \gets sum_2 + value_2$
%		\State $\eta^{-1} \gets 0$
%		\For{$l=1$ \textbf{to} $n_4$}
%		\State $\left(\xinv{l},w^{(l)} \right) \sim \bel{\Xinv}$
%		\For{$m=1$ \textbf{to} $n_5$}
%		\State $\xnew{l,m} \sim \FT(\Xnew \mid \xinv{l}, a)$
%		\State $value \gets w^{(l)} \frac{1}{n_5} \FZ^{(l,m,k)}$
%		\State $\eta^{-1} \gets \eta^{-1} + value$
%		\EndFor
%		\EndFor
%		\State $value_3 \gets w^{(i)} \frac{1}{n_2} \frac{1}{n_3} \log \eta^{-1}$
%		\State $sum_3 \gets sum_3 + value_3$
%		\EndFor
%		\EndFor
%		\EndFor
%		\State $\miaug{\Xinv}{\Xnew}{\Z} \gets sum_1 + sum_2 - sum_3$
%	\end{algorithmic}
%\end{algorithm}


\begin{wrapfigure}{r}{6.8cm}	
	%\centering
	%\includegraphics{std}
	\vspace{-35pt}
	\begin{minipage}{0.95\textwidth}
		\begin{algorithm}[H]
			\caption{\mismc}
			\label{alg:invmi-smc}
			\scriptsize
			\begin{algorithmic}[1]
				\Require $\bel{\Xinv}$, $\FT$, $\FZ$, $a$
				\Ensure $\miaug{\Xinv}{\Xnew}{\Z}$
				\State $sum_1 \gets 0$
				\State $sum_2 \gets 0$
				\State $sum_3 \gets 0$
				\For{$i=1$ \textbf{to} $n_1$}
				\State $\left(\xinv{i},w^{(i)} \right) \sim \bel{\Xinv}$
				\For{$j=1$ \textbf{to} $n_2$}
				\State $\xnew{i,j} \sim \FT(\Xnew \mid \xinv{i}, a)$
				\State $value_1 \gets w^{(i)} \frac{1}{n_2} \log \FT^{(i,j)}$
				\State $sum_1 \gets sum_1 + value_1$
				\For{$k=1$ \textbf{to} $n_3$}
				\State $\zz{i,j,k} \sim \FZ(\Z \mid \xinv{i}, \xnew{i,j})$
				\State $value_2 \gets w^{(i)} \frac{1}{n_2} \frac{1}{n_3} \log \FZ^{(i,j,k)}$
				\State $sum_2 \gets sum_2 + value_2$
				\State $\eta^{-1} \gets 0$
				\For{$l=1$ \textbf{to} $n_4$}
				\State $\left(\xinv{l},w^{(l)} \right) \sim \bel{\Xinv}$
				\For{$m=1$ \textbf{to} $n_5$}
				\State $\xnew{l,m} \sim \FT(\Xnew \mid \xinv{l}, a)$
				\State $value \gets w^{(l)} \frac{1}{n_5} \FZ^{(l,m,k)}$
				\State $\eta^{-1} \gets \eta^{-1} + value$
				\EndFor
				\EndFor
				\State $value_3 \gets w^{(i)} \frac{1}{n_2} \frac{1}{n_3} \log \eta^{-1}$
				\State $sum_3 \gets sum_3 + value_3$
				\EndFor
				\EndFor
				\EndFor
				\State $\miaug{\Xinv}{\Xnew}{\Z} \gets sum_1 + sum_2 - sum_3$
			\end{algorithmic}
		\end{algorithm}
	\end{minipage}
	\vspace{-20pt}
\end{wrapfigure}
%In terms of complexity, the most expensive step of this approach is the estimation of $\ent{\Z}$, thus its complexity is the complexity of the entire estimator. Estimating each ${\eta^{-1}}^{(i,j,k)}$ has a complexity of $O \left( n_4 n_5 d \right)$. In turn, the complexity of estimating $\ent{\Z}$ is of $O \left( n_1 n_2 n_3 n_4 n_5 d \right)$. Considering that we have a total number of $m$ observations instances, i.e. $n_1 n_2 n_3 = m$, and also that the total number of particles is $n$, i.e. $n_4 n_5 = n$, the complexity becomes $O \left( m n d \right)$. In comparison, the complexity of using a re-substitution estimator with KDE is $O \left( m n^2 d \right)$ when using \invmi{}, which makes our estimator favorable in terms of complexity.
Considering that we have a total number of $m$ observations instances and a total number of $n$ particles the complexity becomes $O \left( m n d \right)$. In comparison, the complexity of using a re-substitution estimator with KDE is $O \left( m n^2 d \right)$ when using \invmi{}, which makes our estimator favorable in terms of complexity. The full analysis can be found in Appendix \ref{sec:Complexity}. % section 3.3 in the supplementary material.
We also again emphasize that our estimator avoids the intermediate step of belief surface reconstruction, and hence we conjecture it is expected to be more accurate.

We remind that many more other estimators exist in the literature, and we show in Appendix \ref{sec:Complexity} that \mismc{} is comparable to two of them. Further comparison to additional estimators is left for future research.

%Many other entropy estimators exist in the literature, such as the nearest neighbor estimator, which can be found in \cite{beirlant1997nonparametric}, and the $k$-d partitioning estimator, presented in \cite{stowell2009fast}. When estimating the MI value with these estimators, the complexity
%of both can get to $O \left(m n \log n \right)$, which is comparable to the complexity of \mismc{} when reminding again that $n$ should be exponential in the dimension $d$. We leave further comparison to these additional estimators for future research.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Applicability to Belief Trees}
%

Up to this point, we have shown efficient ways of calculating augmented MI, which is an expectation over the reward, augmented IG. In general, the objective function can then be evaluated through these expected rewards due to commutativity. However, a common solving method, which is to construct a search over a belief-tree, goes through a direct calculation of the reward. The planning literature contains lots of tree-based solvers (e.g. \cite{Sunberg18icaps}, \cite{Fischer20icml}) with which \invmi{} and \mismc{} should be able to cope. Fortunately, we have found that we can define two new rewards, both of which already using \invmi{}, which makes this possible. Meaning, using these new rewards generate the same optimization problem.
For full details and proofs, the reader is refereed to Appendix \ref{sec:AppBeliefTrees}. %Section 4 in the supplementary material.

%Let us shortly denote the original reward, augmented IG, as $\igseq \bydef \igaug{\X_0}{\x_{1:t}}{\Z_{1:t} = \z_{1:t} \mid a_{0:t-1}}$. The first reward which can be used and does not change the optimization problem is its involved counterpart, denoted as $\igseqinv \bydef \igaug{\X_0^{in}}{\x_{1:t}}{\Z_{1:t} = \z_{1:t} \mid a_{0:t-1}}$. This allows to reduce the dimensionality at the reward level, although in general these rewards are not equal (without expectation). \VI{[clarify equal in expectation]}
%
%For the case of \mismc{}, which directly calculates the augmented MI value without going through the calculation of augmented IG, let us denote a consecutive augmented MI between time steps $i-1$ and $i$ as $\micon{i} \bydef \miaug{\X_{i-1}}{x_i}{\Z_i \mid h_i^{-}}$. The second reward is then $\rho_t' = \sum_{i=1}^{t+1} \miconinv{i}$. This reward allows the usage of estimators which directly estimate MI, as our suggested estimator \mismc{} does. We emphasize that \mismc{} will then be used to calculate consecutive augmented MI values.

%\add{While the original reward is $\rho_t = \igaug{\X_0}{\x_{1:t}}{\Z_{1:t} = \z_{1:t} \mid a_{0:t-1}}$, the two equivalent rewards are $\rho_t^{in} = \igaug{\X_0^{in}}{\x_{1:t}}{\Z_{1:t} = \z_{1:t} \mid a_{0:t-1}}$ and $\rho_t' = \sum_{i=1}^{t+1} \miaug{\X_{i-1}}{x_i}{\Z_i \mid h_i^{-}}$. Using the first means that the dimensionality can be reduced also at the reward level, although in general these rewards are equal only in expectation, and not necessarily without it. The second reward allows the usage of estimators which directly estimate MI, as our suggested estimator \mismc{} does.}

%
%In this section we wish to relate the above approaches to the informative planning optimization problem.
%We remind that although the following analysis considers an open-loop formulation, for which we seek  an optimal action sequence, $a_{0:T-1}$, it also applies for a close-loop formulation, for which we seek  a policy, $\pi_{0:T-1}$.
%The solution to the $\rho$-POMDP is obtained by maximization of the objective function. Formulating it recursively yields the Bellman optimality equation
%%
%\begin{equation}
%	\label{eq:bellman_optimality}
%	J_t^{\star} = \underset{a_t}{\max} \left\{ \rho_t + \expec{\ZSp_{t+1}} \left[ J_{t+1}^{\star} \right] \right\},
%\end{equation}
%%
%where $J_t \bydef J \left( \bel{\X_t}, a_{t:T-1} \right)$.
%
%A common solver to this optimization problem is to construct a search over a tree. More specifically, for $\rho$-POMDP, which is the case of belief-dependent rewards, a belief tree is used. In a belief tree, the beliefs $\bel{\X_t}$ are propagated using instances of future actions and observations, then the rewards $\rho_t$ are calculated, and
%the action sequence providing the maximum value for the objective function is eventually chosen.
%Since, in general, the action and observation spaces can be large, in order to be able to solve this optimization problem in reasonable time, it is approximated with a belief tree which propagates only a few sampled instances of future actions and observations. Dealing with continuous such spaces, a belief tree is an approximation of the problem to begin with.
%
%The planning literature contains lots of tree-based solvers (e.g. \cite{sunberg2018online}, \cite{Fischer20icml}) with which we would like our approach, \invmi{}, and our estimator, \mismc{}, to be able to cope. Although our analysis so far was done considering an expected reward, augmented MI, and the optimization problem is based upon the reward itself, an interesting result is that it does not matter. \GR{The full proofs are given in the supplementary material.} Let us shortly denote the original reward, augmented IG, as $\igseq \bydef \igaug{\X_0}{\x_{1:t}}{\Z_{1:t} = \z_{1:t} \mid a_{0:t-1}}$ and its involved counterpart as $\igseqinv \bydef \igaug{\X_0^{in}}{\x_{1:t}}{\Z_{1:t} = \z_{1:t} \mid a_{0:t-1}}$. 
%
%\begin{theorem}
%	\label{th:involved-reward}
%	Let us define the original reward as \( \rho_t = \igseq \) and a new reward, \( \rho_t^{in} = \igseqinv \). Solving the \( \rho \)-POMDP optimization problem with the new reward, \( \rho_t^{in} \), is equivalent to solving it with the original reward, \( \rho_t \), such that
%	\begin{equation}
%		J_t^{\star} = \underset{a_t}{\max} \left\{ \rho_t^{in} + \expec{\ZSp_{t+1}} \left[ J_{t+1}^{\star} \right] \right\}.
%	\end{equation}
%\end{theorem}
%
%This, in turn, means that any optimization solver suitable for the original problem, with the reward $\rho_t$, is also suitable when changing it to $\rho_t^{in}$. This is a key result, since in general these rewards are not equal, however it is much more efficient to calculate $\rho_t^{in}$, as already discussed for the MI case.
%%The belief tree which resembles this new equivalent optimization problem is shown in Figure~\ref{fig:involved_belief_tree_ig}.
%We can then use the IG definition given in eq.~(\ref{eq:augmented_ig_full}) and calculate it through the entropy terms. This result is again general, but the non-parametric setting then necessitate the usage of entropy estimators, plenty of which exist in the literature, as already discussed.
%
%For the case of \mismc{}, which directly calculates the MI value without going through the calculation of IG, let us denote a consecutive MI between time steps $i-1$ and $i$ as $\micon{i} \bydef \miaug{\X_{i-1}}{x_i}{\Z_i \mid h_i^{-}}$.
%
%\begin{theorem}
%	\label{th:involved-expected-reward}
%	Let us define the original reward as \( \rho_t = \igseq \) and a new reward, \( \rho_t' = \sum_{i=1}^{t+1} \miconinv{i} \). Solving the \( \rho \)-POMDP optimization problem with the new reward, \( \rho_t' \), is equivalent to solving it with the original reward, \( \rho_t \), such that
%	\begin{equation}
%		J_t^{\star} = \underset{a_t}{\max} \left\{ \rho_t' + \expec{\ZSp_{t+1}} \left[ J_{t+1}^{\star} \right] \right\}.
%	\end{equation}
%\end{theorem}
%
%This allows the usage of estimators which directly estimate MI, as our suggested estimator \mismc{} does, together with the usage of tree-based solvers of $\rho$-POMDP. However, we emphasize that instead of sequential MI values, we will calculate consecutive MI values.
%
%We note that $\miconinv{i} = \underset{\mathcal{Z}_{i}}{\mathbb{E}}\left[ IG_{i-1}^{i}\right]$. This means that the calculation of the MI values is not limited only to the observations that are used for constructing the tree, thus the calculation can be more accurate, which is another added value of this formulation.
%
%And, lastly, we note that $\rho_t' = \sum_{i=1}^{t+1} \left[ \miconinv{i} \right] = \rho_{t-1}' + I{_{t}^{t+1}}^{in}$. Meaning that for each node, we can calculate the reward based on the previous reward and just update the new information incrementally, without having to calculate the entire reward from scratch.
%The belief tree which resembles this optimization problem is shown in Figure~\ref{fig:involved_belief_tree_mi}.

%Using one-time marginalization, i.e. determining ahead all the involved variables,
%%(together with variables which are required for other reward functions),
%and marginalizing out the rest of the variables, the above analysis suggests that the entire tree can be constructed considering only the marginalized beliefs rather than the entire-state beliefs. This, in turn, reduces also the complexity of constructing this tree, since we avoid maintaining and propagating the beliefs over unnecessary states.

==> 2022 Arxiv/05-Results.tex <==
\graphicspath{ {./Figures/}}

% TODO: split into 2 subsections
% TODO: emphasize what are the actions
% TODO: emphasize the accuracy is only slightly better since we gave an advantage to the KDE

Our approach was tested on an instance of active Simultaneous Localization and Mapping (SLAM) problem, which is a classical choice for high-dimensional problems, since the state contains past trajectory and the map. As in Figure \ref{fig:slam_involved}, an autonomous drone is flying around, observing landmarks which construct a 2D map. At each time step, it needs to decide where to move next in order to reduce its state uncertainty, i.e. the drone's trajectory and the map. In order to make a decision, the drone estimates the augmented MI of the different possible actions at that time. For states which are distributed with Gaussians, the augmented MI can be evaluated using an analytical solution, which makes it a perfect choice as a first validation of our approach. Although Gaussian, we emphasize that the different algorithms get samples as an input, thus work as if it is a purely non-parametric scenario. Using this simulation, we have tested (i) the impact of the dimensionality on choosing an action; and (ii) the impact of increasing the dimensionality on accuracy and timing.

\subsection{Impact of the dimensionality on choosing an action}

At time $t$, the drone needs to choose between four different actions, each involving an observation of a different landmark. In this section, we compare between the analytical solution and the estimation results obtained by three different methods, which we will refer to as \nkde{}, \invmikde{} and \invmismc{}. \nkde{} is the naive approach, which uses a re-substitution estimator with KDE over the entire state; \invmikde{} first uses the \invmi{} approach and only then the re-substitution estimator with KDE, i.e. the estimation is only over the involved subset of the state; \invmismc{} is our suggested estimation scheme, \mismc{}, where we just emphasize that \invmi{} is inherent in it.
We note that for these specific tests, the methods which included KDE were implemented as if the inference engine is perfect, i.e. the posterior samples were generated from the true posterior, whereas \mismc{}, as shown in Algorithm~\ref{alg:invmi-smc}, uses samples from the prior belief and propagates them in a SMC manner. This gives a slight advantage to the methods with KDE over \invmismc{}.
The simulations were done in Python, where we used Scipy's KDE for the two KDE methods.

The prior state has $\sim 150$ dimensions, whereas each action involves a subset of the state with only $4$ dimensions. Each method was provided with $300$ particles (for \invmismc{}, $n_1 = n_4 = 300$, $n_2 = n_3 = n_5 = 1$), and the MI was calculated $100$ times to evaluate its standard deviation. The mean values and standard deviations of each method and for each action are shown in Figure \ref{fig:actions_compare}.
As expected, \nkde{} has big mean errors and big variances. These errors are big enough to make the drone choose an action which isn't optimal. \invmikde{} and \invmismc{}, on the other hand, both present pretty similar and better results compared with \nkde{}, with the former being slightly better in terms of the mean value, probably due to the prior advantage we have provided it with. We note that also for the case of the \invmi{} estimators, the drone might choose an action which isn't optimal due to the similarity between the MI values of this specific test, however an increase in the number of samples will solve this (a smaller increase compared with the one needed for the naive approach).

\begin{figure}
	\centering
	\caption{A comparison between the mean MI values of the different actions and calculation methods. The standard deviation of the calculation methods are shown as error bars. While the mean values, even if not close to the analytical values, maintain action consistency, the real problem is the standard deviation. For a specific trial, the actions ordering might be changed due to the overlaps between MI's possible values. The naive approach suffers the most from this problem.
%		\vspace{-25pt}
}
	\scalebox{0.35}{
		\includegraphics{mean}}
	\label{fig:actions_compare}
%	\vspace{-5pt}
\end{figure}

%\vspace{-5pt}
\subsection{Impact of increasing the dimensionality on accuracy and timing}

We have also tested the impact of increasing state dimensionality on the standard deviation of each estimator, where the action now stays the same.
The original motivation is to show that as the dimension grows, an exponential number of samples would be required in order to get the same accuracy for the naive approach. However, it is not feasible with the dimensions we chose for this simulation. Instead, we approach it in a different manner, and show that as the dimension grows, for a constant number of samples, the accuracy is harmed.
Each estimator, again, was provided with $300$ particles and the MI was calculated $100$ times to evaluate its standard deviation and the average calculation time. The results can be seen in Figure \ref{fig:dimenson_impact}. Both the standard deviation and calculation time of the MI using \nkde{} increase with the state's dimension, an increase which seems linear. On the other hand, for \invmikde{} and \invmismc{} both the standard deviation and calculation time are roughly constant. This is thanks to the fact that the involved subset is of the same dimension during this simulation (only one landmark is observed for each action). This demonstrates our main contribution, for which \invmi{} is better both in terms of accuracy and time complexity, for the same number of samples.
The standard deviation and timing of both \invmikde{} and \invmismc{} are comparable, with a slight advantage to \invmismc{}. We remind that \invmikde{} has a complexity of $O (m n^2 d)$ whereas \invmismc{} has a complexity of $O (m n d)$, which suggests that a better performance should have been obtained for \invmismc{}. However, it is very likely that the Scipy's KDE implementation is optimized, whereas the implementation of \invmismc{} is currently very simple and straightforward. We thus conjecture that the timing could be further improved. We also conjecture that providing the KDE methods with a practical inference engine, rather than the current perfect inference it was provided with, and using more complex distributions, will increase the gap in terms of accuracy.

\begin{figure}
	\centering
	\begin{subfigure}[b]{0.49\textwidth}
		\centering
		\scalebox{0.35}{
			\includegraphics{std}
		}
%		\caption{Standard deviation of MI with increasing state dimensionality}
		\caption{}
		\label{fig:std_with_dimension}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.49\textwidth}
		\centering
		\scalebox{0.35}{
			\includegraphics{time}
		}
%		\caption{Calculation time of MI with increasing state dimensionality}
		\caption{}
		\label{fig:timing_with_dimension}
	\end{subfigure}
	
	\caption{Impact of dimensionality on MSE and calculation time for the three methods. (a) shows the standard deviation, while (b) shows the average calculation time. {\color{blue} \nkde{}}'s error and calculation time both linearly increase with the state's dimension. Using \invmi{} keeps both roughly constant, independent of the state's dimension.
%		\vspace{-25pt}
	}
	\label{fig:dimenson_impact}
	\vspace{-5pt}
\end{figure}

%\begin{figure}
%	\centering
%	\begin{subfigure}[b]{1\textwidth}
%		\centering
%		\scalebox{0.265}{
%			\includegraphics{mean}
%		}
%		\caption{}
%		\label{fig:actions_compare}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}[b]{0.49\textwidth}
%		\centering
%		\scalebox{0.35}{
%			\includegraphics{std}
%		}
%		%		\caption{Standard deviation of MI with increasing state dimensionality}
%		\caption{}
%		\label{fig:std_with_dimension}
%	\end{subfigure}
%	\hfill
%	\begin{subfigure}[b]{0.49\textwidth}
%		\centering
%		\scalebox{0.35}{
%			\includegraphics{time}
%		}
%		%		\caption{Calculation time of MI with increasing state dimensionality}
%		\caption{}
%		\label{fig:timing_with_dimension}
%	\end{subfigure}
%	
%	\caption{(a) A comparison between the mean MI values of the different actions and calculation methods. The standard deviation of the calculation methods are shown as error bars; (b) Impact of dimensionality on the variance; (c) Impact of dimensionality on the calculation time.}
%	\label{fig:dimenson_impact}
%\end{figure}


==> 2022 Arxiv/06-Conclusions.tex <==
%\subsection{Entropy Limitations}
%
%\subsection{Focused}
%
%\subsection{Other}
%Generalization for other costs?
%KL-divergence?
%Efficient high-dimensional inference engine to use with this planner
%Data association not solved

To conclude, we have identified a void in the informative planning subject. For the case of high-dimensional non-parametric beliefs, the complexity becomes too high for solving (not to mention online solutions), thus current state-of-the-art approaches either avoid the high-dimensionality, assume very specific settings or apply rough approximations which impact the accuracy.

In this work, we have filled this void, mainly by reducing the dimensionality of the state for the expected reward's (augmented MI) calculation, while relaxing many of the former assumptions and approximations.
%We have then shown the same conclusion applies also for the more general and complex augmented scenario, in which the dimensionality is inherently increased at each time step. We refer to the approach of dimensionality reduction for MI calculation as \invmi{}.
Next, we have introduced an estimator, \mismc{}, which avoids the reconstruction of future belief's surfaces in case that we have access to the probabilistic models of the problem, which we conjecture might reduce the estimation error and timing, compared to KDE-based approaches, for example. This, in turn, also makes it an anytime algorithm.
Lastly, for the completeness of this work, we have related back to the planning optimization problem and shown how both \invmi{} and \mismc{} can be applied in it.
We emphasize again that this work contributes specifically to the objective function calculation, and thus can be used as a black box together with many other state-of-the-art algorithms which contribute to other building blocks of the planning task.

%Our work was tested on an active SLAM problem, and was compared to a naive approach.
%The results show that \invmi{} is superior to the naive approach of going through the entire state, in terms of both accuracy and timing. \mismc{} is shown to be only slightly better than the KDE estimator, however we conjecture that a code optimization for \mismc{} will increase the gap.

In future work, we would like to extend our approach to the more complex focused case, for which we are only interested in quantifying the uncertainty over a subset of the entire state, as it was done in \cite {Kopitkov17ijrr} for the Gaussian case. Another key aspect that we would like to further investigate is the impact of the non-parametric inference engine in this context. Given the latest novelties in this field, such as the work of \cite{Huang21icra}, we believe it would be very relevant for efficient and accurate non-parametric marginalization.

% TODO
% TODO: limitations:
% Data association assumed to be solved?
% One structue for the observations? (read random sets)
% Differential entropy limitations - actions can be comparable only for states with the same units (i.e. different length trajectories are not comparable with differential entropy. changing units might change the decision)

% TODO
% TODO: future work:
% Simplifications (lower and upper bounds)
% Focused scenario
% Inference engine
% Reward instead of expected reward
% Testing on more complex scenarios (not yet tested on fully non-parametric)
% Could this be generalized to other information-theoretic costs? Even as an approximation...
% Apply ML assumption (or multiple ML observations in case we have a multi-modal belief), or at least a reduction of the number of samples, and check the results
% Check what happens if the belief is represented with multiple data-associations (also into the future, not just in the past)

==> 2022 Arxiv/commands.tex <==

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

%\theoremstyle{definition}
%\newtheorem{example}{Example}[section]


%\definecolor{vadim}{rgb}{1,0.6,0.7}
%\definecolor{shashank}{rgb}{0.6,0.6,1}
%\newcommand{\myputtext}[2]{
	%	\begin{tikzpicture}
		%	\node [fill=#2, rounded corners=2pt] {#1};
		%	\end{tikzpicture}
	%}
%\newcommand{\VI}[1]{\colorbox{vadim}{VI: #1}}
%\newcommand{\SP}[1]{\colorbox{shashank}{SP:#1}}


\newcommand{\VI}[1]{{\color{blue} #1}}
\newcommand{\GR}[1]{{\color{magenta} #1}}
%\newcommand{\GR}[1]{{\color{black} #1}}
% Accepted changes:
\newcommand{\CH}[1]{{\color{green} #1}}
% Added after feedback:
\newcommand{\add}[1]{{\color{red} #1}}


\newcommand{\Zeta}{\mathrm{Z}}
\newcommand{\bydef}{\triangleq}
\newcommand{\bydeff}{\ensuremath{\overset{def}{=}}}
\newcommand{\maxim}[2]{\ensuremath{\underset{#2}{#1}}}
\newcommand{\fnorm}[1]{\ensuremath{{\parallel}#1{\parallel_{\cal F}}}} % this removes spacing, could be ugly for final version
\newcommand{\nrm}[2]{\ensuremath{{\parallel}{#2}{\parallel_{#1}}}}
\newcommand{\nrmsq}[2]{\ensuremath{{\parallel}{#2}{\parallel^2_{#1}}}}
\newcommand{\expt}[2]{\ensuremath{\underset{{#1}}{\mathbb E}{\left\{{#2}\right\}}}}
%\newcommand{\alias}[2]{{#1}\odot{#2}}
\newcommand{\alias}[1]{\ensuremath{\{{#1}\}_{\textbf{aliased}}}}% \xspace}
%\newcommand{\blf}[1]{\ensuremath{b[#1]}}

\newcommand{\prob}[1]{\ensuremath{\mathbb{P}({#1})}}
%\newcommand{\probs}[2]{\ensuremath{\mathbb{P}_{#1}({#2})}}
\newcommand{\blf}[1]{\prob{#1}}

%\usepackage{textcomp,    % for \textlangle and \textrangle macros
%            xspace}
%\newcommand\la{\textlangle\xspace}  % set up short-form macros
%\newcommand\ra{\textrangle\xspace}

%FIXME!
\newcommand\la{\langle\xspace}  % set up short-form macros
\newcommand\ra{\rangle\xspace}

\newcommand*\Let[2]{\State #1 $\gets$ #2}
\algrenewcommand\algorithmicrequire{\textbf{Input:}}
\algrenewcommand\algorithmicensure{\textbf{Input:}}
\algnewcommand{\LineComment}[1]{\State \(\triangleright\) #1}

%new formulation
\newcommand{\priorB}{\ensuremath{\blf{X^-_{k+1}}}\xspace}
\newcommand{\condB}{\blf{X_{k+1} \mid z_{k+1}, \his}\xspace}
\newcommand{\condBi}[1]{\blf{X_{k+1} \mid #1, z_{k+1}, \his}\xspace}
\newcommand{\event}[1]{\ensuremath{A_{#1}}\xspace}

%spaces
\newcommand{\poses}{\ensuremath{{\cal X}}\xspace}
\newcommand{\observations}{\ensuremath{{\cal Z}}\xspace}
\newcommand{\events}{\ensuremath{\{\event{\mathbb{N}}\}}\xspace}
\newcommand{\controls}{\ensuremath{{\cal U}}\xspace}

%history
%\newcommand{\his}{\ensuremath{{\cal H}}\xspace}

%Gilad
\newcommand{\brac}[1]{\ensuremath{\left[ {#1} \right]}}
\newcommand{\augplus}{\ensuremath{\boxplus}}
%Variables
\newcommand{\X}{\ensuremath{X}}
\newcommand{\Xtild}{\ensuremath{\tilde{\X}}}
\newcommand{\his}{\ensuremath{h}}
\newcommand{\Xfut}{\ensuremath{\X'}}
\newcommand{\A}{\ensuremath{A}}
\newcommand{\Z}{\ensuremath{Z}}
\newcommand{\Ztild}{\ensuremath{\tilde{\Z}}}
\newcommand{\ZSp}{\ensuremath{\mathcal{Z}}}
\newcommand{\Xinv}{\ensuremath{\X^{in}}}
\newcommand{\Xinvt}{\ensuremath{\Xtild^{in}}}
\newcommand{\Xinvp}{\ensuremath{\X^{in+}}}
\newcommand{\Xnotm}{\ensuremath{\X^{\neg in-}}}
\newcommand{\Xinvi}[1]{\ensuremath{\X^{in({#1})}}}
\newcommand{\XinvSp}{\ensuremath{\mathcal{\X}^{in}}}
\newcommand{\Xnot}{\ensuremath{\X^{\neg in}}}
\newcommand{\Xnott}{\ensuremath{\Xtild^{\neg in}}}
\newcommand{\Xnew}{\ensuremath{\X_{new}}}
\newcommand{\XnewSp}{\ensuremath{\mathcal{\X}_{new}}}
%Samples
\newcommand{\z}{\ensuremath{z}}
\newcommand{\zz}[1]{\ensuremath{z^{({#1})}}}
\newcommand{\x}{\ensuremath{x}}
\newcommand{\xinv}[1]{\ensuremath{\x^{in({#1})}}}
\newcommand{\xnew}[1]{\ensuremath{\x_{new}^{({#1})}}}
%Definitions
\newcommand{\ent}[1]{\ensuremath{\mathcal{H} \left[ {#1} \right]}}
%\newcommand{\expec}[2]{\ensuremath{\mathbb{E}_{#1} \left[ {#2} \right]}}
\newcommand{\expec}[1]{\ensuremath{\underset{{#1}}{\mathbb{E}}}}
%\newcommand{\mi}[1]{\ensuremath{I \left[ {#1} \right]}}
\newcommand{\ig}[2]{\ensuremath{IG \left[ {#1} ; {#2} \right]}}
\newcommand{\igaug}[3]{\ensuremath{IG_{aug} \left[ {#1} \augplus {#2} ; {#3} \right]}}
\newcommand{\mi}[2]{\ensuremath{I \left[ {#1} ; {#2} \right]}}
\newcommand{\micond}[3]{\ensuremath{I \left[ {#1} ; {#2} \mid {#3} \right]}}
\newcommand{\miaug}[3]{\ensuremath{I_{aug} \left[ {#1} \augplus {#2} ; {#3} \right]}}
\newcommand{\igseq}{\ensuremath{IG_0^t}}
\newcommand{\igseqinv}{\ensuremath{IG{_0^t}^{in}}}
\newcommand{\miseq}{\ensuremath{I_0^t}}
\newcommand{\miseqinv}{\ensuremath{I{_0^t}^{in}}}
\newcommand{\micon}[1]{\ensuremath{I_{{#1}-1}^{#1}}}
\newcommand{\miconinv}[1]{\ensuremath{I{_{{#1}-1}^{#1}}^{in}}}
\newcommand{\FT}{\ensuremath{\mathcal{P}_T}}
\newcommand{\FZ}{\ensuremath{\mathcal{P}_Z}}
\newcommand{\bel}[1]{\ensuremath{b \brac{{#1}}}}
%\newcommand{\bel}[1]{\ensuremath{b \left[ {#1} \right]}}
\newcommand{\dint}{\ensuremath{d\Xnew d\Xinv d\Z}}

% Algorithms
\algrenewcommand\algorithmicrequire{\textbf{Input:}}
\algrenewcommand\algorithmicensure{\textbf{Output:}}

% Names
\newcommand{\invmi}{\texttt{involve-MI}}
\newcommand{\smc}{\texttt{SMC}}
\newcommand{\mismc}{\texttt{MI-SMC}}
\newcommand{\invmismc}{\texttt{involve-MI-SMC}}
\newcommand{\kde}{\texttt{KDE}}
\newcommand{\invmikde}{\texttt{involve-MI-KDE}}
\newcommand{\ann}{\texttt{ANN}}
\newcommand{\kdtree}{\texttt{k-d}}

\newcommand{\nkde}{\texttt{Naive KDE}}


==> 2022 Arxiv/packages.tex <==


\usepackage[english]{babel}
\usepackage[utf8]{inputenc}

%\usepackage{hyperref}

\usepackage[dvipsnames]{xcolor}
\usepackage{color,xcolor,ucs}
%\usepackage{color,xcolor}

%\usepackage{mathptmx}       % selects Times Roman as basic font
%\usepackage{subfig}
\usepackage{floatrow}
\usepackage{tabularx}
\usepackage{float}
\usepackage{amsfonts}
%\usepackage{helvet}         % selects Helvetica as sans-serif font
%\usepackage{courier}        % selects Courier as typewriter font
%\usepackage{type1cm}        % activate if the above 3 fonts are
% not available on your system
\usepackage{amsmath}
% using for \triangleq
% from http://tex.stackexchange.com/questions/151670/latex-symbol-for-leftrightarrow-with-triangleq
\usepackage{amssymb}
%
\usepackage{makeidx}         % allows index generation
\usepackage{comment}         % allows index generation
\usepackage{graphicx}        % standard LaTeX graphics tool
% when including figure files
\usepackage{multicol}        % used for the two-column index
\usepackage[bottom]{footmisc}% places footnotes at page bottom
\usepackage{bm}

\usepackage{cite}
\usepackage{url}

%\usepackage[bookmarks=true]{hyperref}


%\usepackage[unicode=true, bookmarks=true,colorlinks=true]{hyperref}
\usepackage{xr-hyper}


%\usepackage[linesnumbered, inoutnumbered]{algorithm2e}
%\usepackage{algpseudocode,algorithm,algorithmicx}
\usepackage{algorithm}
\usepackage{algpseudocode}



\usepackage{xspace}
\usepackage{rotating}

%\usepackage{tikz}
%\usepackage{pgfplots}
%\usepackage{tkz-graph}
%\usetikzlibrary{arrows,shapes,shadows,positioning,calc}


\usepackage{graphicx}
\usepackage{threeparttable}
\usepackage{multirow}
\usepackage[font=scriptsize,labelfont=bf]{caption}

\usepackage{subcaption}
\captionsetup{compatibility=false}

\usepackage{wrapfig}

\usepackage[title]{appendix}
%\usepackage{titlesec}
%\titlespacing*{\section}
%{0pt}{5.5ex plus 1ex minus .2ex}{4.3ex plus .2ex}
%\titlespacing*{\subsection}
%{0pt}{5.5ex plus 1ex minus .2ex}{2.3ex plus .2ex}

%\usepackage{eucal}

==> 2022 Arxiv/title.tex <==
%\title{\invmi{}: Informative Planning with High-Dimensional Non-Parametric Beliefs}
%
%\author{%
%	Gilad Rotman\thanks{MSc Student, TASP, gilad.rotman@gmail.com.}
%	\and
%	Vadim Indelman\thanks{Associate Professor, Faculty of Aerospace Engineering, vadim.indelman@technion.ac.il.}\\
%	{\normalsize\itshape
%		Technion Israel Institute of Technology, Haifa, 3200003, Israel}
%}

%\title{\invmi{}: Informative Planning with High-Dimensional Non-Parametric Beliefs\thanks{This work was partially supported by the Israel Science Foundation (ISF) and by US NSF/US-Israel BSF.}}
%
%%\titlerunning{Informative Planning with High-Dimensional Non-Parametric Beliefs}
%
%\author{Gilad Rotman \and
%	Vadim Indelman}
%
%\institute{Technion -- Israel Institute of Technology, Haifa, 3200003, Israel,
%		\email{gilad.rotman@campus.technion.ac.il}, %\\
%		\email{vadim.indelman@technion.ac.il}\\
%		%Home page: \url{vindelman.net.technion.ac.il}
%}


%
\title{\LARGE \bf \invmi{}: Informative Planning with High-Dimensional Non-Parametric Beliefs\thanks{This work was partially supported by the Israel Science Foundation (ISF) and by US NSF/US-Israel BSF.}}
%

\author{Gilad Rotman$^{1}$ and Vadim Indelman$^{2}$ \\
	$^1$Technion Autonomous Systems Program (TASP) \\
	$^2$Department of Aerospace Engineering\\
	Technion - Israel Institute of Technology, Haifa 32000, Israel\\
	\small{\texttt{gilad.rotman@technion.ac.il, vadim.indelman@technion.ac.il}}}



\date{}


%%
%\title{Contribution Title\thanks{Supported by organization x.}}
%%
%%\titlerunning{Abbreviated paper title}
%% If the paper title is too long for the running head, you can set
%% an abbreviated paper title here
%%
%\author{First Author\inst{1}\orcidID{0000-1111-2222-3333} \and
%	Second Author\inst{2,3}\orcidID{1111-2222-3333-4444} \and
%	Third Author\inst{3}\orcidID{2222--3333-4444-5555}}
%%
%\authorrunning{F. Author et al.}
%% First names are abbreviated in the running head.
%% If there are more than two authors, 'et al.' is used.
%%
%\institute{Princeton University, Princeton NJ 08544, USA \and
%	Springer Heidelberg, Tiergartenstr. 17, 69121 Heidelberg, Germany
%	\email{lncs@springer.com}\\
%	\url{http://www.springer.com/gp/computer-science/lncs} \and
%	ABC Institute, Rupert-Karls-University Heidelberg, Heidelberg, Germany\\
%	\email{\{abc,lncs\}@uni-heidelberg.de}}
%%
%\maketitle              % typeset the header of the contribution
%%
